Annealed Importance Sampling with q-Paths

Annealed importance sampling (AIS) is the gold standard for estimating partition functions or marginal likelihoods, corresponding to importance sampling over a path of distributions between a tractable base and an unnormalized target. While AIS yields an unbiased estimator for any path, existing literature has been primarily limited to the geometric mixture or moment-averaged paths associated with the exponential family and KL divergence. We explore AIS using $q$-paths, which include the geometric path as a special case and are related to the homogeneous power mean, deformed exponential family, and $\alpha$-divergence.

==> sections/3_info_geo.tex <==
\section{Information Geometric Interpretation}
%%%%%%

Information geometry concerns the study of differential geometric structures over the space of probability distributions $\mathcal{P}$ or unnormalized measures $\mathcal{M}_+$ \cite{amari2016information, nielsen2018elementary}.  In this section, we explore the statistical manifolds induced by the $\alpha$-paths described above. 





%\citet{eguchi1983second} : from divergence to manifold

%In $\mathbb{R}^n$, $D_{\alpha}$ appears to be dually flat ( or \citet{amari2016information} 4.1.2)
%an also try restricting to parametric distributions in the $q$-exponential family
% Following the recipe of \citet{eguchi1983second}, one can use any divergence measure to derive a dual pair of affine connections $\nabla, \nabla^{*}$, which define a covariant derivative operator and parallel transport of vectors between neighboring tangent spaces.   Along with a metric tensor $g$, this defines an \textit{information manifold} $(\mathcal{P}, g, \nabla, \nabla^{*})$. 


% The \textsc{kl} divergence defines a dually flat information manifold $(\mathcal{P}, g^F, \nabla^{1}, \nabla^{-1})$
% \begin{itemize}
% \item \textcolor{red}{Does? } the variational representation \eqref{eq:vrep} corresponds to the distributions along the $\nabla^{(-1)}$ geodesic curve between $f_0$ and $f_T$, parameterized by $t$ (i.e. reverse \textsc{kl}, $\mathbb{E}_{i} D_{\psi}[\theta_i : \theta]$).  (similarly for the reverse \textsc{kl}, with geodesic for connection $\nabla^{(1)}$ )
% \end{itemize}



% $D_{\alpha}$  induces a dually flat structure $(\mathcal{M}_+, g^{?}, \nabla^{(\alpha)}, \nabla^{(-\alpha})$
% \paragraph{Interpreting this:}
 
% \item TO DO : what is the metric $g$?   (Fisher on $\mathcal{M}_+$?) %(simplify \citet{zhang2004divergence} Prop. 7? or even Euclidean (\citet{amari2016information} Sec. 3.6) ))

% \item as above, would hope to interpret $\alpha$-path as a geodesic with respect to $(\mathcal{M}_+, g, \nabla^{\alpha}, \nabla^{-\alpha})$?

% \begin{itemize}
%     \item Can we have dually flat structure on an $\infty$-dim space?
% \begin{itemize}
%     \item \citet{zhang2004divergence} Sec. 3.2 (Ex. 3.2.1, Prop 6) appears to have the same form as the canonical divergence (i.e. $D[\theta : \eta] = \psi(\theta) + \psi^{*}(\eta) - \theta \cdot \eta$)
%     \item \citet{zhang2004divergence} restrict to finite-dim parameter vectors $\theta_p$, $\theta_q$ to define dually flat structure (Prop 7)
%     \item In $\mathbb{R}^n$, $D_{\alpha}$ appears to be dually flat (\citet{felice2019canonical} or \citet{amari2016information} 4.1.2)
% \end{itemize}

% \end{itemize}




% Compare to $\pm \alpha$ connections induced by $D_{KL} = D_{\pm 1}$ as in \citet{nielsen2018elementary}?
% \begin{itemize}
% \item i.e. $\nabla^{\alpha} = \frac{1-\alpha}{2} \nabla^{(-1)} + \frac{1+\alpha}{2} \nabla^{(1)}$
% \item  unsure... ( haven't taken third derivatives)   
% \item  would be nice to be able to unify $\alpha$-paths as $\alpha$-connection induced by $D_{KL} = D_{\pm 1}$
% \end{itemize}


% $\alpha$-path (after normalization) matches the $q$-geodesic in $q$-exponential family (\cite{amari2011geometry} Eq. 65, App. \ref{app:breg_table})
% \begin{itemize}
%     \item even though $q$-geometry is over normalized $\mathcal{P}$, has $g_{ij} = \frac{1}{Z(\text{escort})} g_{ij}^{\text{Fisher}}$ as metric
% \end{itemize}

%Path for $D_{\alpha}$ (in $\mathcal{M}_+$) matches that of $q$-exponential family ( \citet{amari2011geometry}(see \cref{app:breg_table})?
% \begin{itemize}
%     \item $q$-exp family and $\alpha$-mean have same intermediate \textit{unnormalized} densities, different geometry (over different spaces)
%     \item i.e. $q$ geometry constructed using flat divergence over \textit{normalized} distributions (based on normalizer $\psi_q$)
% \end{itemize}

==> sections/app/breg_table.tex <==
\section{Comparison of Exponential Family and $q$-Exponential Family}\label{app:breg_table}
\begin{table}[h]
\centering
\caption{\label{tab:properties}}
\begin{tabular}{p{2cm} p{6.1cm} p{6.5cm}} % \cmidrule(r){1-1}
  \cmidrule(lr){2-2} \cmidrule(l){3-3} \\[.25ex]
 & Exponential Family ($q=1$) & $q$-Exponential Family \\ \midrule
Definition & $\pi_{\beta}(\z) = \pi_0(\z) \, \exp \{ \beta \cdot \phi(\z) - \psi(\beta) \}$  & $\pi_{\lambda}(\z) = \pi_0(\z) \, \exp_q \{ \lambda \cdot \phi(\z) - \psi_q(\lambda) \} $ \\[2ex]
Free Energy & $\psi(\beta)  = \ln Z_{\beta} $ & $\psi_q(\lambda)$ \\[2ex]
Escort Dist. & $\Pi_{\beta, 1} =  \pi_0(\z)^{1-1} \, \pi_{\beta}(\z)^1 =  \pi_{\beta}(\z)  $ & $ \Pi_{\lambda,q} = \dfrac{1}{z_{q}(\lambda)} \pi_0(\z)^{1-q} \, \pi_{\lambda,q}(\z)^q $ \\[2ex]
Dual Params 		& $\dfrac{\partial \psi(\beta)}{\partial \beta^j} = \eta^j =  \mathbb{E}_{\pi_{\beta}}[\phi_j(\z)]$    \, (standard)		& $\dfrac{\partial \psi_q(\lambda)}{\partial \lambda^j} =\eta^j_q =\mathbb{E}_{\Pi_{\lambda,q}}[\phi_j(\z)] $ \, (escort) \\[2ex]
Bregman Div. & $D_{\psi}[\beta^{\prime} : \beta ] = D_{KL}[ \pi_{\beta} || \pi_{\beta^{\prime}} ] $ & $D_{\psi_q}[\lambda^{\prime} : \lambda ] = \mathbb{E}_{\Pi_{\lambda, q} }[ \ln_q \dfrac{\pi_{\lambda,q}}{\pi_0} - \ln_q \dfrac{\pi_{\lambda^{\prime},q}}{\pi_0}] $ \\[2ex]
& $\phantom{D_{\psi}[\beta^{\prime} : \beta ]} = \mathbb{E}_{\pi_{\beta}} [ \ln \pi_{\beta} - \ln \pi_{\beta^{\prime}} ]$ &  \\[2ex]
Conjugate $\psi^{*}$ & $\psi^{*}(\eta) = D_{\psi}[\pi_0 ||  \pi_{\beta_{\eta}}] =D_{KL}[\pi_{\beta_{\eta}}||\pi_0 ] $ & $\psi_q^{*}(\eta) = D_{\psi_q}[\pi_0 ||\pi_{\lambda_{\eta},q}] = \mathbb{E}_{\Pi_{\lambda, q} }[ \ln_q \dfrac{\pi_{\lambda_{\eta},q}}{\pi_0} ] $\\[2ex] 
& & $\phantom{\psi_q^{*}(\eta) = } \hfill = \dfrac{1}{1-q}\bigg(\dfrac{1}{z_q(\lambda)} -1 \bigg) $ \\[3.5ex] \\
Neg. Entropy & $\psi^{*}(\eta) = \mathbb{E}_{\pi_{\beta_{\eta}}}[ \log \pi_{\beta_{\eta}} ] $\footnotesize \quad (if $\pi_0 =$uniform)& $\psi_q^{*}(\eta) = \mathbb{E}_{\Pi_{\lambda, q}}[ \ln_q \pi_{\lambda_{\eta},q} ] $  \footnotesize \quad (if $\pi_0 = $uniform) \\[3ex]
\small Dual Definition & $\pi_{\beta}(\z) = \pi_0(\z) \exp \{ \beta \, ( \phi(\z) - \eta ) + \psi^{*}(\eta) \}$  & $\pi_{\lambda}(\z) = \pi_0(\z)\exp_q \{ \lambda \, ( \phi(\z) - \eta_q ) + \psi_q(\lambda) \}$ \\
\bottomrule
\end{tabular}
\end{table}


==> sections/app/geo.tex <==
\newcommand{\alphaainv}{{\frac{2}{1-\alpha}}}
\newcommand{\alphaa}{{\frac{1-\alpha}{2}}}
\newcommand{\alphaaneg}{{\frac{1+\alpha}{2}}}
\newcommand{\alphaaneginv}{{\frac{2}{1+\alpha}}}

\section{\citet{zhang2013nonparametric} Geodesics }
This section closely follows \citet{zhang2013nonparametric} Sec. 2.2-2.3.
We will seek to show that our $q$-path
\begin{align}
    \ln_q \big(\tpi_{t, q}(z)\big) = (1-t) \ln_q \big(\tpi_{0}(z)\big) + t \, \ln_q \big(\tpi_{1}(z) \big)
\end{align}
forms a geodesic for the affine connection induced by the $\alpha$-divergence $D_{\alpha}$ over unnormalized measures.


Consider the $\rho, \tau$ embeddings
\begin{align}
    \rho(\tpi(z)) =  \alphaainv \big( \tpi(z)^\alphaa - 1 \big) \qquad \tau(\tpi) = \alphaaneginv  \big( \tpi(z)^\alphaaneg - 1 \big)
\end{align}
which are conjugate with respect to the function 
\begin{align}
    f(\rho) = \alphaaneginv \big( 1 + \alphaa \cdot \rho)^\alphaainv
\end{align}
where conjugacy means that $\tau(\tpi(z)) = f^{\prime}\big(\rho(\tpi(z))\big)$.


This induces a family of $\alpha$-divergences $D^{(\alpha)}_{f,\rho}$, where $\alpha$ is intended to reflect \textit{referential duality}.   Our use of $\alpha$ in the $\rho, \tau$ embedding functions, or $q$ in the $\ln_q$ path, rather reflects \textit{representational duality} in terms of the $\alpha$-representation (e.g. \citet{amari2010divergencefunctions}).   

% geodesic is wrt second argument
We obtain the flat divergence, which integrates an expression of Bregman form
\begin{align}
    D^{(1)}_{f, \rho}[\tpi_a:\tpi_b] =  \int f\big(\rho(\tpi_a(z)) \big) -  f\big(\rho(\tpi_b(z)) \big) + \big( \rho(\tpi_a(z)) - \rho(\tpi_b(z)) \big) \cdot  \tau(\tpi_b) dz
\end{align}
which can be shown to correspond to Amari's $\alpha$ divergence for the choice of $f, \rho$ above.
\begin{align}
D^{(1)}_{f, \rho}[\tpi_a:\tpi_b] &= D_{\alpha}[\tpi_a(\vz):\tpi_b(\vz) ] \\
&= \frac{4}{(1-\alpha^2)} \bigg( \frac{1-\alpha}{2}  \int \tpi_a(\vz) \,d\vz +  \frac{1+\alpha}{2}  \int \tpi_b(\vz) \,d\vz -\int \tpi_a(\vz)^{\frac{1-\alpha}{2}} \, \tpi_b(\vz)^{\frac{1+\alpha}{2}}  d\vz  \bigg)
\end{align}
As shown in Proposition 2 and Corollary 3 of \citet{zhang2013nonparametric}, we can define an information manifold $(\mathcal{M}_+, g_{ij}^{(D^{(1)}_{f,\rho})}, \nabla^{(1)}, \nabla^{(-1)})$.   See \citet{zhang2013nonparametric} for additional details.   We consider only the affine connection $\nabla^{(1)}$ in what follows, which is a special case of the $\alpha$-connection for the above manifold
\begin{align*}
    \nabla^{(\alpha)}_{\dot{\gamma}} \dot{\gamma} = (d_{\dot{\gamma}} \dot{\gamma})_{\gamma_t} + \frac{d}{d\gamma} \big( \alphaaneg \log \rho^{\prime}(\gamma(t)) + \alphaa \log \tau^{\prime}(\gamma(t)) \big) \label{eq:affine_alpha}
\end{align*}



\subsection{$q$-Path as Geodesic}
Our $q$-path distributions $\tpi_{t, q}$ along a curve parameterized by $t$, are defined using the power mean with function $\rho(u)$, and are thus linear in the $\rho$ representation
\begin{align}
    \rho\big( \gamma(t)\big) = \rho\big(\tpi_{t, q}(z)\big) = (1-t) \rho\big(\tpi_{0}(z)\big) + t \, \rho\big(\tpi_{1}(z) \big)
\end{align}
where $\rho(u) = \ln_q(u)$ for $q = 2\alpha-1$. %(see Eq. \eqref{eq:lnqexpq}).

We seek to show that our $q$-path is a geodesic with respect to the affine connection $\nabla^{(1)}$, or an autoparallel path.  Let $\gamma_t = \gamma(t) = \tpi_{t,q}(z)$ indicate the $q$-path distribution with mixing parameter $t$, with $\dot{\gamma} = d \gamma_t / dt$.  

Plugging $\alpha = 1$ into \eqref{eq:affine_alpha} , and with $ (d_{\dot{\gamma}} \dot{\gamma})_{\gamma_t} = \frac{d \dot{\gamma(t)}}{d\gamma_t} \cdot \dot{\gamma}$ , we seek to show that $\nabla_{\dot{\gamma}} \dot{\gamma} = 0$, or
\begin{align*}
    \nabla^{(1)}_{\dot{\gamma}} \dot{\gamma} = \frac{d \dot{\gamma}}{d\gamma} \cdot \dot{\gamma} + \big(\dot{\gamma}\big)^{2} \cdot \frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) 
\end{align}


We will first derive several useful quantities.  Since it is easier to differentiate $\rho(\gamma(t)) = (1-t) \rho(\tpi_0) + t \, \rho(\tpi_1)$ with respect to $\gamma$, we note that $\frac{d}{dt} \rho\big( \gamma(t) \big) = \frac{d \rho(\gamma) }{d\gamma(t)} \frac{d\gamma(t)}{dt}$.  We can then rewrite the desired $\frac{d\gamma(t)}{dt}$ as 
\begin{align}
    \dot{\gamma} = \frac{d\gamma(t)}{dt} &= \bigg( \frac{d \rho(\gamma_t) }{d\gamma(t)} \bigg)^{-1} \, \frac{d \rho(\gamma_t) }{dt} = \gamma^{\alphaaneg} \cdot \big( \rho(\tpi_1) - \rho(\tpi_0) \big) \\[1.4ex]
    \implies  \dot{\gamma} &=\gamma_t \cdot \big( \rho(\tpi_1) - \rho(\tpi_0) \big) \quad (\text{for $\alpha = 1$}) \label{eq:dgamma_dt}
\end{align}
since 
\begin{align}
    \frac{d \rho(\gamma_t) }{d\gamma_t}  &= \frac{d}{d \gamma_t} \alphaainv \big( \gamma^\alphaa - 1 \big) = \gamma_t^{\alphaa - \frac{2}{2}} =  \gamma_t^{\frac{-(1+\alpha)}{2}} \\
    \text{and } \quad \frac{d \rho(\gamma_t) }{dt}  &= \frac{d}{dt} \big( (1-t) \rho(\tpi_0) + t \, \rho(\tpi_1) \big) = \rho(\tpi_1) - \rho(\tpi_0)
\end{align}

We can now differentiate the $\frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) $ term in the affine connection.   From above, $d \rho(\gamma_t) / d\gamma(t) = \gamma_t^{\frac{-(1+\alpha)}{2}}$, so that
\begin{align}
    \frac{d}{d\gamma} \big(  \log \frac{d}{d\gamma} \rho(\gamma(t)) \big) &=   \frac{d}{d\gamma}   \log \big( \gamma_t^{\frac{-(1+\alpha)}{2}} \big) = -\frac{(1+\alpha)}{2} \cdot \frac{d}{d\gamma}   \log \gamma_t \\
    &\phantom{\frac{d}{d\gamma}   \log \big( \gamma_t^{\frac{-(1+\alpha)}{2}} \big)} = -\frac{(1+\alpha)}{2} \gamma_t^{-1} \\
    % &= \gamma_t^{\frac{(1+\alpha)}{2}} \cdot \frac{d}{d\gamma} \gamma_t^{\frac{(1+\alpha)}{2}} \\
    % % &=
    % % \bigg( \frac{d}{d\gamma} \rho(\gamma_t) \bigg)^{-1} \cdot \frac{d}{d\gamma}  \rho(\gamma_t) \\
    % &= \gamma^{\frac{(1+\alpha)}{2}} \cdot  - \frac{(1+\alpha)}{2} \gamma^{-\frac{(1+\alpha)}{2}-1} \\
    % &= -\gamma_t \cdot \gamma_t^{-2} \\
    \implies \frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) &=  -\gamma_t^{-1} \quad (\text{for $\alpha=1$}) \label{eq:db_dgamma}
\end{align}


Putting it all together, and with dot products turning into scalar products for our one-dimensional curve $t$, we have
\begin{align}
    \nabla^{(1)}_{\dot{\gamma}} \dot{\gamma} &=  \frac{d \dot{\gamma}}{d\gamma_t} \cdot \dot{\gamma}  + \big(\dot{\gamma}\big)^{2} \frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) \\
    &=  \frac{d }{d\gamma_t} \bigg( \gamma_t \cdot \big( \rho(\tpi_1) - \rho(\tpi_0) \big) \bigg) \cdot \dot{\gamma}  -  (\dot{\gamma})^{2} \gamma_t^{-1}
    \qquad \quad \text{(using \eqref{eq:dgamma_dt} and \eqref{eq:db_dgamma})} \\
    &= \dot{\gamma} \cdot \big( \rho(\tpi_1) - \rho(\tpi_0) \big) - (\dot{\gamma})^{2} \cdot {\dot{\gamma}}^{-1} \cdot \big( \rho(\tpi_1) - \rho(\tpi_0) \big) \qquad \text{(rearranging \eqref{eq:dgamma_dt})} \\
    &= \dot{\gamma} \cdot \big( \rho(\tpi_1) - \rho(\tpi_0) \big) - \dot{\gamma} \cdot \big( \rho(\tpi_1) - \rho(\tpi_0) \big) \\
    &=0
\end{align}

\clearpage
\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_01.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_09.pdf}}
    \subfigure[$q=0.9$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_18.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_20.pdf}}
    \subfigure[$q=1.1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_12_redo.pdf}}
    \subfigure[$q=1.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_2_redo.pdf}} 
    \subfigure[$q=2$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_3_redo.pdf}}%
    \subfigure[$q=3$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_4_redo.pdf}}
    \caption{Intermediate densities between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$ for various $q$-paths and 10 equally spaced $\beta$. The path approaches a mixture of Gaussians with  weight $\beta$ at $q=0$.  For the geometric mixture ($q=1$), intermediate $\pi_{\beta}$ stay within the exponential family since both $\pi_0$, $\pi_T$ are Gaussian.}
    \label{fig:alpha_path} 
    \vspace*{-.15cm}
\end{figure}


\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha-1_student_df2_2.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha05_student_df2_2.pdf}}
    \subfigure[$q=0.95$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha95_student_df2_2.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha1_student_df2_2.pdf}}
    \subfigure[$q=1.1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha11_student_df2_2.pdf}}
    \subfigure[$q=1.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha15_student_df2_2.pdf}} 
    \subfigure[$q=2$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha2_student_df2_2.pdf}}%
    \subfigure[$q=3$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha3_student_df2_2.pdf}}
    \caption{Intermediate densities between $\text{Student}(\text{df}=2, -4, 3)$ and $\text{Student}(\text{df}=2, 4, 1)$ for various $q$-paths and 10 equally spaced $\beta$.}
    \label{fig:q_path} 
    \vspace*{-.15cm}
\end{figure}



\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha-1_student_df2_2.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha05_student_df2_2.pdf}}
    \subfigure[$q=0.95$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha95_student_df2_2.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha1_student_df2_2.pdf}}
    \subfigure[$q=1.1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha11_student_df2_2.pdf}}
    \subfigure[$q=1.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha15_student_df2_2.pdf}} 
    \subfigure[$q=2$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha2_student_df2_2.pdf}}%
    \subfigure[$q=3$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha3_student_df2_2.pdf}}
    \caption{Tail behavior for densities between $\text{Student}(\text{df}=2, -4, 3)$ and $\text{Student}(\text{df}=2, 4, 1)$ for various $q$-paths and 10 equally spaced $\beta$.}
    \label{fig:q_path} 
    \vspace*{-.15cm}
\end{figure}

==> sections/app/vm_naudts_paths.tex <==
\section{Derivation of Path $q$-Family}\label{app:q_path}
With normalization, the $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
\begin{align}
    \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ \eta \cdot \phi(\vz) - \psi_q(\eta)  \big\} \label{eq:lnq_fam_form1}
\end{align}
which is suggestive of the convex conjugate for $\psi_q$ via
\begin{align}
    \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  \eta \cdot \phi(\vz) - \psi_q(\eta)
\end{align}
We now derive the $q$-exponential family from the $\alpha$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.

\begin{proof}
\begin{align}
    \pi_{\alpha, \beta}(z) &\propto \bigg[(1 - \beta) \pi_0^{1 - \alpha} + \beta\pi_1^{1 - \alpha}\bigg]^\frac{1}{1 - \alpha}\\
    &= \bigg[\pi_0^{1 - \alpha} + \beta\big(\pi_1^{1 - \alpha} - \pi_0^{1 - \alpha}\big)\bigg]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + \beta\left(\left(\frac{\pi_1}{\pi_0}\right)^{1 - \alpha} - 1\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + (1-\alpha)\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \exp_\alpha\left[\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right].
\end{align}
Defining $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$ and normalizing, we arrive at
\begin{align}
    \pi_{\alpha, \beta}(z) = \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \quad
    Z_\alpha(\beta) &:= \int dz \pi_0 \exp_\alpha\left[\beta \phi(\vz) \right].\label{eq:lnq_fam_form2}
\end{align}

To get \cref{eq:lnq_fam_form2} into the standard $q$-exponential family form, we define
\begin{align}
    \psi_\alpha := \ln_\alpha^* \left(Z_\alpha(\beta)\right) \label{eq:psi_alpha}
\end{align}
and rewrite \cref{eq:lnq_fam_form2} using \cref{eq:q_exp_prod}
\begin{align}
    \pi_{\alpha, \beta}(z) &= \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \\
    &= \frac{\pi_0}{\exp^*_\alpha\left(\psi_\alpha\right)}\exp_\alpha\left(\beta \phi(\vz) \right) & \text{Using  \cref{eq:psi_alpha}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha\right) \exp_\alpha\left(\beta \phi(\vz)\right) & \text{Using $\exp^*_\alpha(u) = 1/\exp_\alpha(-u)$}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \bigg(1 - (1 - \alpha) \psi_\alpha\bigg)\beta\phi(\vz)\right) & \text{Using \cref{eq:q_exp_prod}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \eta \phi(\vz)\right)
\end{align}
where we have defined
\begin{align}
    \eta := \beta \cdot \big(1 - (1 - \alpha) \psi_\alpha\big).
\end{align}
\end{proof}



\section{Alternative Derivation}
Note that $\exp_q \{ x + y \} = \exp_q \{ y \} \cdot \exp_q \{ \frac{x}{1 + (1-q) y}  \}$ from \textcolor{red}{Vaden's theorem below.}, instead of $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $ for the standard exponential.  This implies that
\begin{align}
\pi_{q,\beta} = \pi_0 \, \exp_q \{ \beta \cdot \phi(\vz) - \psi_q \} &= \pi_0 \, \exp_q\{ -\psi_q \} \exp_q \{ \frac{\beta}{1+(1-q)(-\psi_q)} \cdot \phi(\vz) \} 
\end{align}
Our goal is to express $\pi_{q,\beta}(\vz)$ using a normalization constant $Z$ instead of the $q$-free energy $\psi_q(\beta)$.  While the exponential family allows us to freely move between  $\log Z_{\beta}$
and $\psi(\beta)$, in the $q$-exponential case, we must adjust the parameters.   Defining
%To (w/ $\eta, \beta$ switched) match Naudts, let : }
\begin{align}
 \eta &= \frac{\beta}{1+(1-q)(-\psi_q)} \\
Z_q(\eta) &= \frac{1}{\exp_q \{-\psi_q \}} := \exp_{q}^{*}\{ -\psi_q\} \\
\end{align}
we obtain a new parameterization of the $q$-exponential family, using parameters $\eta$ and multiplicative normalization constant $Z_q(\eta)$, as
\begin{align}
 \pi_{q,\beta} =  \pi_{q,\eta} &=  \frac{1}{Z_q(\eta)} \exp_{q} \{ \eta \cdot \phi(\vz) \}
\end{align}
See \citet{matsuzoe2019normalization} for more detailed discussion of normalization in deformed exponential families.


==> sections/app/vm_q_sum_prod.tex <==
\section{Sum and Product Identities for $q$-Exponentials}\label{app:q_sum_product}
In this section, we prove two lemmas which are useful for manipulation expressions involving $q$-exponentials, for example in moving between \cref{eq:normalization1} and \cref{eq:normalization2} in either direction.
\begin{lemma}
    Sum identity
    \begin{align}
        \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
    \end{align}
    \label{lemma:q_exp_sum}
\end{lemma}
\begin{lemma}
    Product identity
    \begin{align}
        \prod_{n=1}^N \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1 - q)x_i\right)\right)\label{eq:q_exp_prod}
    \end{align}
    \label{lemma:q_exp_prod}
\end{lemma}

\subsection{Proof of \cref{lemma:q_exp_sum}}
\begin{proof}
    We prove by induction. The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$ so that the denominator on the \textsc{rhs} of \cref{eq:q_exp_sum} is $1$. Assuming \cref{eq:q_exp_sum} holds for $N$,
    \begin{align}
        \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \left[ 1 + (1-q) \sum_{n=1}^{N+1} x_n \right]_{+}^{1/(1-q)} \\
                                                &= \left[ 1 + (1-q) \left(\sum_{n=1}^{N} x_n\right) + (1-q)x_{N+1} \right]_{+}^{1/(1-q)} \\
                                                &= \left[\left( 1 + (1-q) \sum_{n=1}^{N} x_n \right) \left(1 + (1-q)\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n}\right) \right]_{+}^{1/(1-q)} \\
                                                &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n} \right)\\
                                                &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + (1-q)\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
    \end{align}
\end{proof}
\subsection{Proof of \cref{lemma:q_exp_prod}}
\begin{proof}
    We prove by induction. The base case ($N=1$) is satisfied using the convention $\prod_{i=a}^bx_i = 1$ if $b < a$. Assuming \cref{eq:q_exp_prod} holds for $N$, we will show the $N+1$ case. To simplify notation we define $y_N:=\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + = (1 - q)x_i\right)$. Then, 
    %and $(1-q) = (1 - q)$. Then
\begin{align}
    \prod_{n=1}^{N+1} \exp_q(x_n) &= \exp_q(x_{1})\left(\prod_{n=2}^{N+1}\exp_q(x_n)\right)\\
    &= \exp_q(x_{0})\left(\prod_{n=1}^{N}\exp_q(x_n)\right) & \hspace*{-.5cm} \text{(reindex $n \to n - 1)$} \nonumber \\
    &=\exp_q(x_{0})\exp_q(y_N) & \hspace*{-.5cm} \text{(inductive hypothesis)} \nonumber \\
    &= \bigg[\left(1 + (1-q) \cdot x_{0}\right)\left(1 + (1-q) \cdot y_N\right) \bigg]_{+}^{1/(1-q)}\\
    &= \bigg[1 + (1-q) \cdot x_{0} + \big(1 + (1-q) \cdot x_{0} \big)(1-q) \cdot y_N \bigg]_{+}^{1/(1-q)}\\
    &= \bigg[1 + (1-q) \bigg(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)y_N\bigg) \bigg]_{+}^{1/(1-q)}\\
    &= \exp_q \left(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)y_N\right)
\end{align}
Next we use the definition of $y_N$ and rearrange
\begin{align}
    &= \exp_q \left(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)\left(x_1 + x_2(1 + (1-q) \cdot x_1) + ... + x_N \cdot \prod_{i=1}^{N-1}(1 + (1-q) \cdot x_i)\right)\right) \nonumber\\
    &= \exp_q\left(\sum_{n=0}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1-q) x_i\right)\right).
\end{align}
Then reindexing $n \to n + 1$ establishes
\begin{align}
    \prod_{n=1}^{N+1} \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N+1}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1-q)x_i\right)\right).
\end{align}
\end{proof}


% \section{Sum Identity for $q$-exponentials}\label{app:q_sum_product}
% %\section{Sum and product identities for $q$-exponentials}\label{app:q_sum_product}
% While the exponential family has the convenient property that $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $, this is not true for $\exp_{\alpha}\{ x + y \}$.   We derive a more general expression for the $q$-exponential below.
% %In the Lemma below, prove a more general statement for the $q$-exponential.
% %We therefore derive two lemmas for q-exponentials which will be useful in obtaining the $q$-exponential family. We will prove both statements by induction and simplify notation by defining $(1-q) := 1 - q$.

% \begin{lemma}
%     Sum identity
%     \begin{align}
%         \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
%     \end{align}
%     \begin{proof}
%         The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$ so that the denominator on the \textsc{rhs} of \cref{eq:q_exp_sum} is $1$. Assuming \cref{eq:q_exp_sum} holds for $N$,
%         \begin{align}
%             \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \bigg[ 1 + (1-q) \sum_{n=1}^{N+1} x_n \bigg]^{1/(1-q)} \\
%                                                     &= \bigg[ 1 + (1-q) \left(\sum_{n=1}^{N} x_n\right) + (1-q)x_{N+1} \bigg]^{1/(1-q)} \\
%                                                     &= \bigg[\left( 1 + (1-q) \sum_{n=1}^{N} x_n \right) \left(1 + (1-q)\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n}\right) \bigg]^{1/(1-q)} \\
%                                                     &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n} \right)\\
%                                                     &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + (1-q)\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
%         \end{align}
%     \end{proof}
% \end{lemma}

% %\section{Sum and product identities for $q$-exponentials}\label{app:q_sum_product}
% While the exponential family has the convenient property that $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $, this is not true for $\exp_{\alpha}\{ x + y \}$. We therefore derive two lemmas for q-exponentials which will be useful in obtaining the $q$-exponential family. We will prove both statements by induction and simplify notation by defining $\bar{q} := 1 - q$.

% \begin{lemma}
%     Sum identity
%     \begin{align}
%         \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
%     \end{align}
%     \begin{proof}
%         The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$. Assuming \cref{eq:q_exp_sum} holds for $N$,
%         \begin{align}
%             \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \bigg[ 1 + \bar{q} \sum_{n=1}^{N+1} x_n \bigg]^{1/\bar{q}} \\
%                                                     &= \bigg[ 1 + \bar{q} \left(\sum_{n=1}^{N} x_n\right) + \bar{q}x_{N+1} \bigg]^{1/\bar{q}} \\
%                                                     &= \bigg[\left( 1 + \bar{q} \sum_{n=1}^{N} x_n \right) \left(1 + \bar{q}\frac{x_{N+1}}{1 + \bar{q} \sum_{n=1}^{N} x_n}\right) \bigg]^{1/\bar{q}} \\
%                                                     &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + \bar{q} \sum_{n=1}^{N} x_n} \right)\\
%                                                     &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + \bar{q}\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
%         \end{align}
%     \end{proof}
% \end{lemma}

% \begin{lemma}
%     Product identity
%     \begin{align}
%         \prod_{n=1}^N \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1 - q)x_i\right)\right)\label{eq:q_exp_prod}
%     \end{align}
%     \begin{proof}
%         The base case ($N=1$) is satisfied using the convention $\prod_{i=a}^bx_i = 1$ if $b < a$. Assuming \cref{eq:q_exp_prod} holds for $N$, we will show the $N+1$ case. To simplify notation we define $y_N:=\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q}x_i\right)$. Then
%     \begin{align}
%         \prod_{n=1}^{N+1} \exp_q(x_n) &= \exp_q(x_{1})\left(\prod_{n=2}^{N+1}\exp_q(x_n)\right)\\
%         &= \exp_q(x_{0})\left(\prod_{n=1}^{N}\exp_q(x_n)\right) & \text{(reindex $n \to n - 1)$}\\
%         &=\exp_q(x_{0})\exp_q(y_N) & \text{(inductive hypothesis)}\\
%         &= \bigg[\left(1 + \bar{q} \cdot x_{0}\right)\left(1 + \bar{q} \cdot y_N\right) \bigg]^{1/\bar{q}}\\
%         &= \bigg[1 + \bar{q} \cdot x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)\bar{q} \cdot y_N \bigg]^{1/\bar{q}}\\
%         &= \bigg[1 + \bar{q} \bigg(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)y_N\bigg) \bigg]^{1/\bar{q}}\\
%         &= \exp_q \left(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)y_N\right)
%     \end{align}
%     Next we use the definition of $y_N$ and rearrange
%     \begin{align}
%         &= \exp_q \left(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)\left(x_1 + x_2(1 + \bar{q} \cdot x_1) + ... + x_N \cdot \prod_{i=1}^{N-1}(1 + \bar{q} \cdot x_i)\right)\right)\\
%         &= \exp_q\left(\sum_{n=0}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q} x_i\right)\right).
%     \end{align}
%     Then reindexing $n \to n + 1$ establishes
%     \begin{align}
%         \prod_{n=1}^{N+1} \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N+1}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q}x_i\right)\right).
%     \end{align}
% \end{proof}
% \end{lemma}







% \section{Derivation of Path $q$-Family}\label{app:q_path}
% \vm{This longer derivation is necessary to establish relationship between two q-exp fam forms and allow for tvo/ti trick. Might also be better to save for full paper and revert to prev}
% With normalization, the $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
% \begin{align}
%     \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ \eta \cdot \phi(\vz) - \psi_q(\eta)  \big\} \label{eq:lnq_fam_form1}
% \end{align}
% which is suggestive of the convex conjugate for $\psi_q$ via
% \begin{align}
%     \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  \eta \cdot \phi(\vz) - \psi_q(\eta)
% \end{align}
% We now derive the $q$-exponential family from the $\alpha$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.

% \begin{proof}
% \begin{align}
%     \pi_{\alpha, \beta}(z) &\propto \bigg[(1 - \beta) \pi_0^{1 - \alpha} + \beta\pi_1^{1 - \alpha}\bigg]^\frac{1}{1 - \alpha}\\
%     &= \bigg[\pi_0^{1 - \alpha} + \beta\big(\pi_1^{1 - \alpha} - \pi_0^{1 - \alpha}\big)\bigg]^\frac{1}{1 - \alpha}\\
%     &= \pi_0 \left[1 + \beta\left(\left(\frac{\pi_1}{\pi_0}\right)^{1 - \alpha} - 1\right)\right]^\frac{1}{1 - \alpha}\\
%     &= \pi_0 \left[1 + (1-\alpha)\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right]^\frac{1}{1 - \alpha}\\
%     &= \pi_0 \exp_\alpha\left[\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right].
% \end{align}
% Defining $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$ and normalizing, we arrive at
% \begin{align}
%     \pi_{\alpha, \beta}(z) = \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \quad
%     Z_\alpha(\beta) &:= \int dz \pi_0 \exp_\alpha\left[\beta \phi(\vz) \right].\label{eq:lnq_fam_form2}
% \end{align}

% To get \cref{eq:lnq_fam_form2} into the standard $q$-exponential family form, we define
% \begin{align}
%     \psi_\alpha := \ln_\alpha^* \left(Z_\alpha(\beta)\right) \label{eq:psi_alpha}
% \end{align}
% and rewrite \cref{eq:lnq_fam_form2} using \cref{eq:q_exp_prod}
% \begin{align}
%     \pi_{\alpha, \beta}(z) &= \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \\
%     &= \frac{\pi_0}{\exp^*_\alpha\left(\psi_\alpha\right)}\exp_\alpha\left(\beta \phi(\vz) \right) & \text{Using  \cref{eq:psi_alpha}}\\
%     &= \pi_0 \exp_\alpha\left(-\psi_\alpha\right) \exp_\alpha\left(\beta \phi(\vz)\right) & \text{Using $\exp^*_\alpha(u) = 1/\exp_\alpha(-u)$}\\
%     &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \bigg(1 - (1 - \alpha) \psi_\alpha\bigg)\beta\phi(\vz)\right) & \text{Using \cref{eq:q_exp_prod}}\\
%     &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \eta \phi(\vz)\right)
% \end{align}
% where we have defined
% \begin{align}
%     \eta := \beta \cdot \big(1 - (1 - \alpha) \psi_\alpha\big).
% \end{align}
% \end{proof}


==> sections/bkup/pre_vaden_thursday_night/0_intro.tex <==
\section{Introduction}
% We generalize the geometric and moment-averaged paths used to interpolate between a base distribution $\tpi_0$ and target $\tpi_T$ in methods such as annealed importance sampling (\gls{AIS}).

% The moment-averaged path \cite{grosse2013annealing} can be difficult to calculate outside of tractable exponential families \vm{Does this make sense? Is it even \textit{defined} outside of exponential families?} and may require additional sampling procedures to approximate.
%   While \citet{GelmanPathSampling-1998} derive expressions for optimal annealing paths, \textit{these appear similarly intractable} for annealing between arbitrary distributions.

%   Our proposed $\alpha$-mixture path provides a closed form expression for intermediate unnormalized densities, which, like the geometric mixture path, may be used directly as the energy function for common \gls{MCMC} transition operators.

\gls{AIS} \cite{neal2001annealed, jarzynski1997equilibrium} is a method for estimating intractable normalization constants, which considers a path of intermediate distributions between a tractable base distribution $\pi_0(\vz)$ and unnormalized target $\tpi_T(\vz)$.  In particular, \gls{AIS} samples from a sequence of \textsc{mcmc} transition operators $\mathcal{T}_{t}(\vz_{t}|\vz_{t-1})$, which leave each $\pi_t(\vz) = \tpi_t(\vz)/ Z_{t} $ invariant, to estimate the ratio $Z_T / Z_0$.   
% Writing intermediate distributions as %$\pi_{t}(\vz) & = \frac{\tpi_t(\vz)}{Z_{t}} $ with $ Z_{t} = \int \tpi_t(\vz) \, d\vz,$
% \begin{align}
%     \pi_{t}(\vz) & = \frac{\tpi_t(\vz)}{Z_{t}} & &Z_{t} = \int \tpi_t(\vz) \, d\vz, \label{eq:arbitrary_path} 
% \end{align}
As shown in \cref{alg:ais}, we can accumulate the importance weights $w_{T}^{(i)} = \prod_{t=1}^{T} \tpi_t(z_{t - 1}) / \tpi_{t-1}(z_{t - 1})$ along the path and take the expectation of $w_{T}^{(i)}$ over sampling chains to obtain an unbiased estimate of $Z_T  / Z_0$ \cite{neal2001annealed}.  Similarly, \gls{BDMC} \cite{grosse2015sandwiching, grosse2016measuring} provides lower and upper bounds on the \textit{log} partition function ratio $\log Z_T / Z_0$ using \gls{AIS} initialized with the base or target distribution, respectively.  

% we can accumulate the importance weights $w_{T}^{(i)} = \prod_{t=1}^{T} \tpi_t(z_{t - 1}) / \tpi_{t-1}(z_{t - 1})$ along the chain as shown in \cref{alg:ais}. %\limits
% Taking the expectation of $w_{T}^{(i)}$ over chains yields an unbiased estimate of $Z_T  / Z_0$ \cite{neal2001annealed}, while \gls{BDMC} \cite{grosse2015sandwiching, grosse2016measuring} provides lower and upper bounds on the \textit{log} partition function ratio $\log Z_T / Z_0$ using \gls{AIS} initialized with the base or target distribution, respectively.  
\gls{AIS} commonly uses a geometric mixture path parameterized by $\{ \beta_t \}_{t=0}^T$  to interpolate between $\pi_0$ at $\beta_0 = 0$, and $\tpi_1$ at $\beta_T = 1$, 
\begin{align}
    \pi_{t}(\vz) & = \frac{\tpi_0(\vz)^{1-\beta_t} \, \tpi_T(\vz)^{\beta_t}}{Z_{\beta_t}} & &Z_{t} = \int \tpi_0(\vz)^{1-\beta_t} \tpi_T(\vz)^{\beta_t} d\vz, \label{eq:geopath} 
    %\\ \pi^{(q)}_{\beta_t}(\vz) & = \frac{\tpi^{(q)}_{\beta_t}(\vz)}{Z^{(q)}_{\beta_t}} \quad \quad \text{where } Z^{(q)}_{\beta_t} = \int \tpi_\beta(\vz) d\vz \label{eq:geopath2}
\end{align}

%\cite{grosse2013annealing}(see Sec. \ref{sec:alpha_paths}, App. \ref{app:grosse_alpha}), 
Alternative paths have been discussed in \cite{grosse2013annealing,gelman1998simulating, thang}, but may not have closed form expressions for $\tpi_t(\vz)$.   In this work, we propose to generalize the geometric mixture path \eqref{eq:geopath} using the \textcolor{red}{{\abstractmean}} \cite{kolmogorov1930,hardy1953, de2016mean, amari2007integration}, or $q$-path, 
\begin{align}
    % \tpi^{(\alpha)}_\beta &= \bigg( (1-\beta) \, \tpi_0^{\frac{1-\alpha}{2}} + \beta \, \tpi_T^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}} \label{eq:alpha_mix0}\\
    \tpi^{(q)}_{t}(\vz) &= \bigg( (1-\beta_t) \, \tpi_0(\vz)^{1-q} + \beta_t \, \tpi_T(\vz)^{1-q} \bigg)^{\frac{1}{1-q}}  \label{eq:alpha_mix0} \\
    Z^{(q)}_{t} &= \int \tpi^{(q)}_{t}(\vz) d\vz, \nonumber
    % & &Z^{(q)}_{t} = \int \tpi^{(q)}_{t}(\vz) d\vz, \label{eq:alpha_mix0}
\end{align}
%In Sec. \ref{sec:geo} and \ref{sec:alpha_paths}, we provide several ways of understanding how these paths generalize the geometric mixture path, which is recovered as $q\rightarrow 1$ and is associated with the $\log$ mixture, exponential family, and variational representations based on the \textsc{kl} divergence (\citet{grosse2013annealing}).

As $q\rightarrow 1$, we recover the geometric mixture path as a special case.   In Sec. \ref{sec:alternative_interpretations}, we associate the geometric path with the $\log$ mixture, exponential family, and variational representations based on the \textsc{kl} divergence \cite{grosse2013annealing}, in order to prepare for our analogous discussion of the $q$-path in Sec. \ref{sec:alpha_paths}.

%We provide additional insights into the correspondence between the \abstractmean, 

Our use of the order parameter $q$ reflects direct connections with the deformed logarithm in non-extensive thermodynamics \cite{tsallis1988possible, naudts2011generalised, tsallis2009introduction}, while our construction is also intimately related to the $q$-exponential family \cite{amari2011q} and $\alpha$-geometry of \citet{amari1982differential} \cite{amari2007integration,amari2016information}.  In particular, we show that our $q$-path \eqref{eq:alpha_mix0} can be given a variational representation using the $\alpha$-divergence over unnormalized measures \cite{amari2007integration}.
%where $q$ is written to indicate  




% Similarly, the $\alpha$ path can be interpreted using
% \begin{itemize}
%     \item $\ln_q$ mixtures or abstract means
%     \item $\alpha$- or $q$-exponential family
%     \item variational representation of $\alpha$-divergence
% \end{itemize}

% where the \textsc{kl} divergence corresponds to $\alpha \pm 1$.

%intermediate distributions $\pi_t(\vz) = \tpi_t(\vz)/ Z_{t}$ for ${t = 0, 1, ..., T}$ to estimate the ratio of normalization constants $Z_T / Z_0$





% In particular, we propose paths using the $\alpha$-mean of unnormalized densities $\tpi^{(\alpha)}_\beta$ for $\beta \in [0,1]$, $\alpha \neq 1$
% \begin{align}
%     % \tpi^{(\alpha)}_\beta &= \bigg( (1-\beta) \, \tpi_0^{\frac{1-\alpha}{2}} + \beta \, \tpi_T^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}} \label{eq:alpha_mix0}\\
%     \tpi^{(q)}_{t} &= \bigg( (1-\beta_t) \, \tpi_0(\vz)^{1-q} + \beta_t \, \tpi_T(\vz)^{1-q} \bigg)^{\frac{1}{1-q}} \label{eq:alpha_mix0}
% \end{align}
% with $\lim \limits_{\alpha \rightarrow 1} \tpi^{(\alpha)}_t = \exp \big( (1-\beta) \, \log \tpi_0 + \beta \, \log \tpi_T  \big)$ corresponding to the geometric mixture. \vm{mmmmmmm q form looks so good}







% \section{Background}
% \subsection{Annealed Importance Sampling}
% \gls{AIS} \citep{neal2001annealed, jarzynski1997equilibrium} considers a path of intermediate distributions $\pi_{\beta_t}(\vz) \propto \tpi_{\beta_t}(\vz)$ connecting a tractable base distribution $\pi_0 (\vz) = \tpi_0(\vz)/ Z_0$ and a target $\pi_T(\vz) = \tpi_T(\vz) / Z_T$, with the goal of estimating the ratio of normalization constants $Z_T / Z_0$.
% %Commonly, \gls{AIS} considers a geometric mixture path parameterized by $t$
% \begin{align}%\beta_
%     \pi_{\beta}(\vz) & = \frac{\tpi_{\beta}(\vz)}{Z_{\beta}} \quad \quad \text{where } Z_{\beta} = \int \tpi_\beta(\vz) d\vz \label{eq:geopath}
% \end{align}
% \gls{AIS} proceeds to construct \gls{MCMC} transition operators, which leave each intermediate distribution invariant, $\pi_{\beta_t}(\vz) = \int T(\vz | \vz') \, \pi_{\beta_t}(\vz') d\vz'$ and yield a sequence of samples $\vz_t$.   For example, using \gls{HMC} \cite{neal2011mcmc, betancourt2017geometric}), we only need access to the energy function $\log \tpi_\beta$.

% Interpreting each $\vz_t$ as a proposal for an importance sampling estimate of $\tpi_{t+1}(\vz_t) / \tpi_t(\vz_t) $, we can accumulate the importance weights along a chain as $ w_{0:T-1} $ .  Taking the expectation
% % \begin{align}
% %     w_{0:T-1} = \prod \limits_{t=0}^{T-1}  \dfrac{\tpi_{t+1}(\vz_{t})}{\tpi_{t}(\vz_{t})}  \, . \label{eq:ais_weights} %= \exp \big\{  - \sum \limits_{t=0}^{T-1} (\beta_{t+1}-\beta_{t}) \cdot \E (\vz_{t})  \big \} \label{eq:ais_weights}
% % \end{align}
% yields an unbiased estimator of the partition function ratio (see, for example, \cite{neal2001annealed, grosse2015sandwiching, habeck2017model})
% \begin{align}
%     \frac{Z_T}{Z_0} = \mathbb{E}_{\vz_{0:T-1}}[ w_{0:T-1} ] \approx \frac{1}{N} \sum \limits_{i=1}^N w^{(n)}_{0:T-1} \qquad \text{where  }   w_{0:T-1} = \prod \limits_{t=0}^{T-1}  \dfrac{\tpi_{t+1}(\vz_{t})}{\tpi_{t}(\vz_{t})}
% \end{align}
% For example,  we may be interested in estimating the marginal likelihood $Z_T = p_{\theta}(\vx) = \int p_{\theta}(\vx, \vz) d\vz$ in a generative model, with the unnormalized target $\tpi_T = p_{\theta}(\vx, \vz)$ corresponding to the joint density.  %Starting from a base distribution or prior $\tpi_0(\vz)$, each \gls{AIS} path will yield a unique estimator of $p_{\theta}(\vx)$.



% \section{Annealed Importance Sampling}
% Given a tractable base distribution $\pi_0 (\vz) = \tpi_0(\vz)/ Z_0$ and an intractable target distribution $\pi_T(\vz) = \tpi_T(\vz) / Z_T$,
% \gls{AIS} \citep{neal2001annealed, jarzynski1997equilibrium} uses a path of intermediate distributions $\pi_t(\vz) = \tpi_t(\vz)/ Z_{t}$ for ${t = 0, 1, ..., T}$ to estimate the ratio of normalization constants $Z_T / Z_0$.
% To form the intermediate distributions \gls{AIS} commonly uses a geometric path, parameterized by $\beta$, to gradually ``anneal'' between reference and target
% \begin{align}
%     \pi_{\beta}(\vz) & = \frac{\tpi_0(\vz)^{1-\beta}\tpi_T(\vz)^{\beta}}{Z_{\beta}} & &Z_{\beta} = \int \tpi_0(\vz)^{1-\beta} \tpi_T(\vz)^{\beta} d\vz, \label{eq:geopath} \\
%     \pi^{(q)}_{\beta_t}(\vz) & = \frac{\tpi^{(q)}_{\beta_t}(\vz)}{Z^{(q)}_{\beta_t}} \quad \quad \text{where } Z^{(q)}_{\beta_t} = \int \tpi_\beta(\vz) d\vz \label{eq:geopath2}
% \end{align}
% where a sequence of \gls{MCMC} transition operators $T_t(\vz | \vz')$ with stationary distributions $\pi_{\beta_t}(\vz)$ are used to generate samples along the path.
% Interpreting each $\vz_t \sim  T_t(\vz | \vz_{t-1})$ as a proposal for an importance sampling estimate of $\tpi_{t+1}(\vz_t) / \tpi_t(\vz_t)$, we can accumulate the importance weights along a chain as $w_{0:K-1}$. Taking the expectation w.r.t the path yields an unbiased estimator of the partition function ratio (see App. 1.1 in \cite{habeck2017model} for a detailed derivation)
% \begin{align}
%     \frac{Z_T}{Z_0} = \mathbb{E}_{\vz_{0:T-1}}[ w_{0:T-1} ] \approx \frac{1}{N} \sum \limits_{i=1}^N w^{(n)}_{0:T-1} \qquad \text{where  }   w_{0:T-1} = \prod \limits_{t=0}^{T-1}  \dfrac{\tpi_{t+1}(\vz_{t})}{\tpi_{t}(\vz_{t})}.
% \end{align}
% For example, we may be interested in estimating the marginal likelihood $Z_T = p_{\theta}(\vx) = \int p_{\theta}(\vx, \vz) d\vz$ in a generative model, with the unnormalized target $\tpi_T = p_{\theta}(\vx, \vz)$ corresponding to the joint density. We summarize \gls{AIS} in \cref{alg:ais}.


==> sections/bkup/pre_vaden_thursday_night/1_geopath.tex <==
\section{Interpretations of the Geometric Path}\label{sec:alternative_interpretations}
\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_01.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_09.pdf}}
    \subfigure[$q=0.9$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_18.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_20.pdf}}
    \caption{Intermediate densities using various $q$-paths between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$, with 10 equally spaced $\beta_t$. The $q$-path approaches a mixture of Gaussians with mixing parameter $\beta$ at $q=0$, and becomes a geometric mixture parameterized by $\beta$ at $q=1$.}
    \label{fig:alpha_path}
\end{figure}
\begin{wrapfigure}{r}{0.35\textwidth}
    \begin{minipage}{0.35\textwidth}
        \vspace{-15pt}
        \begin{algorithm}[H]
            \SetAlgoLined
                \For{i = 1 \text{to} N}{
                $z_0 \sim \pi_0(z)$\\
                $w^{(i)} \leftarrow Z_0$\\
                % $w_ \leftarrow Z_0$\\
                \For{t = 1 to T}{
                $w_t^{(i)} \leftarrow$ $w_t^{(i)} \frac{\tpi_t(z_{t - 1}^{(i)})}{\tpi_{t-1}(z_{t - 1}^{(i)})}$\\
                $z_t^{(i)} \sim T_t(\vz_t | \vz_{t-1}^{(i)})$\\ %^{(i)}
                }
                }
                \Return{$Z_T / Z_0 \approx \frac{1}{N} \sum_N w_t^{(i)}$}
                \caption{Annealed IS}
                \label{alg:ais}
        \end{algorithm}
        % \captionof{algorithm}{Annealed Importance Sampling}
    \end{minipage}
    \vspace{-30pt}
  \end{wrapfigure}

In this section, we give three complementary interpretations of the geometric path defined in \cref{eq:geopath}, which will have generalized analogues in \cref{sec:alpha_paths}.
% We construct the geometric mixture path using the unnormalized densities as in \eqref{eq:geopath} %We let $\tpi_t$ denote unnormalized densitities, with $\pi_t$ indicating the corresponding distribution normalized by $Z_t$.
% \begin{align}%\beta_
%     \pi_{t}(\vz) & = \frac{\tpi_{t}(\vz)}{Z_{t}} = \frac{\tpi_0(\vz)^{1-t} \, \tpi_T(\vz)^{t}}{Z_{t}} \quad \quad \text{where: } Z_{t} = \int \tpi_0(\vz)^{1-t} \tpi_T(\vz)^{t} d\vz \label{eq:geopath}
% \end{align}

\paragraph{Log Mixture} 
Simply taking the logarithm of both sides of the geometric mixture \eqref{eq:geopath} shows that $\tpi_t$ can be obtained by taking the log-mixture of $\tpi_0$ and $\tpi_T$ with mixing parameter $\beta_t$,

%The simplest alternative interpretation is that of a log-mixture between $\tpi_0$ and $\tpi_T$, which may be obtained by taking the logarithm of both sides of \cref{eq:geopath}
\begin{align}
%\pi_\beta(\vz) \propto \exp\big\{(1-\beta)\log \tpi_0(\vz) + \beta\log \tpi_T(\vz) \}.
% \pi_\beta(\vz) = \exp\big\{(1-\beta)\log \tpi_0(\vz) + \beta\log \tpi_T(\vz) - c\big\},
\log \tpi_t (\vz) = (1-\beta_t) \, \log \tpi_0(\vz) + \beta_t \, \log \tpi_T(\vz)
\end{align}

where we may also choose to subtract a constant $c = \log Z_t = \psi(\beta_t)$ to enforce normalization.
% where $c = \log Z_t$ accounts for normalization.

\paragraph{Exponential Family} Distributions along the geometric path may also be viewed as coming from an exponential family \cite{brekelmans2020tvo}. In particular, we use a base measure of $\tpi_0(\vz)$ and sufficient statistics $\phi(\vz) = \log \tpi_T / \tpi_0$ to rewrite $\tpi_{\beta_t} = \tpi_0(\vz)^{1-\beta_t} \, \tpi_T(\vz)^{\beta_t}$ as 
\begin{align}
    \pi_{t}(\vz) &= \tpi_0(\vz) \, \exp \{ \beta_t \cdot \log \frac{\tpi_T(\vz)}{\tpi_0(\vz)} - \psi(\beta_t) \}  =\frac{1}{Z_{\beta_t}} \tpi_0(\vz) \, \exp \{ \beta_t \cdot \log \frac{\tpi_T(\vz)}{\tpi_0(\vz)}\}  \label{eq:exp_fam} %= \frac{1}{Z_{\beta_t}} \tpi_0(\vz)^{1-\beta_t} \, \tpi_T(\vz)^{\beta_t} } 
\end{align}
where the mixing parameter $\beta_t$ appears as the natural parameter of the exponential family. The log-partition function or free energy $\psi(\beta_t)$, which is convex in $\beta_t$, suggests a dual pair of Bregman divergences over the natural parameter space which reduce to the \textsc{kl} divergence \cite{amari2016information, nielsen2018elementary, brekelmans2020tvo}
%is defined $\psi(\beta) = \log \int  \tpi_0(\vz) \, \exp \{ \beta \cdot \log \frac{\tpi_T(\vz)}{\tpi_0(\vz) } \} d\vz$.

%Since the log partition function $\psi(\tau)$ is a convex function of $\tau$, we can construct a Bregman divergence $D_{\psi}[t : t^{\prime}] $ between intermediate distributions along this path.   For any exponential family, this divergence corresponds to the \textsc{kl} divergence between distributions indexed by $t$ and $t^{\prime}$,
% \begin{align}
%     D_{\psi}[t : t^{\prime}] = \psi(t) - \psi(t^{\prime}) - \langle t- t^{\prime} , \nabla \psi(t) \rangle = D_{KL}[\pi_{t^{\prime}}(\vz) || \pi_{t}(\vz) ]
% \end{align}
% where $\langle \cdot, \cdot \rangle$ indicates a dot product, which reduces to a product for our one-dimensional parameter $t$.

\paragraph{Variational Interpretation} %also
Similarly, \citet{grosse2013annealing} observe that each $\pi_{\beta}(\vz)$ can be viewed as minimizing a weighted sum of \textsc{kl} divergences to the (normalized) base and target distributions %the distribution
\begin{align}
    \pi_{\beta}(\vz) &= \argmin \limits_{r(\vz)} (1-\beta) \, D_{KL}[ r(\z) || \pi_{0}(\vz)] + \beta D_{KL}[  r(\z) || \pi_{T}(\vz)] \label{eq:vrep}.
\end{align}
While the optimization \eqref{eq:vrep} is over arbitrary $r(\vz)$, the optimal distribution is the geometric mixture with mixing parameter $\beta$, which is a member of the exponential family \eqref{eq:exp_fam} (see Sec. \ref{sec:alpha_paths} or App. \ref{app:alpha_integration}). %with $\log$ likelihood ratio sufficient statistic.  
%\vm{pointer to \rb{where?} ... App. \ref{app:mixture_path} in section 3.5}

%The moment averaged path of \citet{grosse2013annealing} is obtained as the solution to an analogous variational objective using the reverse \textsc{kl} divergence. \vm{will point to App. \ref{app:mixture_path} in section 3.5}

% move to later
% , although this optimization is only over distributions on the geometric mixture path \eqref{eq:exp_fam} or within a parametric family.  We discuss this distinction in App. \ref{app:mixture_path}.


%but this optimization is only over distributions in a parametric family. We discuss this distinction in App. \ref{app:mixture_path}. % Sec. \ and

%In App. \ref{app:breg_info}, we interpret this result using a general result about Bregman divergences from \citet{Banerjee2005}, where the expected Bregman divergence to a single point $\mu$ in the second argument is minimized by the mean over arguments $\mu = (1-t) \cdot 0 + t \cdot T = t \cdot T$.  With $T=1$, we have $t\cdot T = t$.

% \subsection{Moment-Averaged Path}
% \begin{itemize}
%     \item Introduce conjugate $\psi^{*}$, moments $\eta$, dual divergence $D_{\psi^{*}}$
%     \item Moments-averaged path of \citet{grosse2013annealing} as variational representation using $D_{\psi^{*}}$
% \end{itemize}

% From the convexity of the log partition function $\psi(\tau)$, one can consider its convex conjugate $\psi^{*}$
% \begin{align}
% \psi^{*}(\eta) = \sup_{\tau} \tau \cdot \eta - \psi(\tau) \qquad \implies \eta_j &= \frac{\partial \psi}{\partial \tau} \label{eq:conjugate}  \label{eq:conjugate}
% \end{align}
% where $\eta = \{ \eta_j \}$ and $\tau = \{ \tau_j \}$ may correspond to $J > 1$ sufficient statistics $\phi(\vz) = \{\phi_j(\vz)\}$.

% Since $\psi(\tau)$ is convex, its gradient will be unique and increasing at each $\tau$.   We can thus use $\eta = \nabla \psi(\tau)$ as a \textit{dual} way of parameterizing a distribution in the exponential family.  In particular,
% \begin{align}
%     \eta_j &= \frac{\partial \psi}{\partial \tau} = \mathbb{E}_{\pi_{\tau}}[ \phi_j(\vz) ] \, \, \forall \, \, j
% \end{align}
% which corresponds to the supremum in \eqref{eq:conjugate}.


% \subsection{Alternative Interpretations }\label{sec:geo}
% In this section, we give three complementary interpretations of the geometric mixture path defined in \ref{eq:geopath}, which will mirrored in our generalizations in \cref{sec:alpha_paths}.

% % We construct the geometric mixture path using the unnormalized densities as in \eqref{eq:geopath} %We let $\tpi_t$ denote unnormalized densitities, with $\pi_t$ indicating the corresponding distribution normalized by $Z_t$.
% % \begin{align}%\beta_
% %     \pi_{t}(\vz) & = \frac{\tpi_{t}(\vz)}{Z_{t}} = \frac{\tpi_0(\vz)^{1-t} \, \tpi_T(\vz)^{t}}{Z_{t}} \quad \quad \text{where: } Z_{t} = \int \tpi_0(\vz)^{1-t} \tpi_T(\vz)^{t} d\vz \label{eq:geopath}
% % \end{align}

% \paragraph{Log Mixture Path} The simplest Simply taking the logarithm of both sides of the geometric mixture \eqref{eq:geopath} shows that $\pi_t$ may be obtained by taking the log-mixture of $\tpi_0$ and $\tpi_T$,
% \begin{align}
% \log \pi_t(\vz) = (1-t) \, \log \tpi_0(\vz) + t \, \log \tpi_T(\vz) - c
% \end{align}
% where $c = \log Z_t$ accounts for normalization.

% \paragraph{Exponential Family:} The geometric- or log-mixture $\pi_t(\vz)$ may also be framed in terms of an exponential family \cite{brekelmans2020tvo}.   In particular, we use a base measure of $\tpi_0(\vz)$ and sufficient statistics $\phi(\vz) = \log \tpi_T / \tpi_0$ to obtain
% \begin{align}
%     \pi_{t}(\vz) = \tpi_0(\vz) \, \exp \{ t \cdot \log \frac{\tpi_T(\vz)}{\tpi_0(\vz)} - \psi(t) \}  \quad \text{where } \, \,  \psi(t) = \log \int  \tpi_0(\vz) \, \exp \{ t \cdot \log \frac{\tpi_T(\vz)}{\tpi_0(\vz) } \} d\vz \label{eq:exp_fam}
% \end{align}
% where the mixing parameter $t$ appears as the natural parameter of the exponential family.

% %Since the log partition function $\psi(\tau)$ is a convex function of $\tau$, we can construct a Bregman divergence $D_{\psi}[t : t^{\prime}] $ between intermediate distributions along this path.   For any exponential family, this divergence corresponds to the \textsc{kl} divergence between distributions indexed by $t$ and $t^{\prime}$,
% % \begin{align}
% %     D_{\psi}[t : t^{\prime}] = \psi(t) - \psi(t^{\prime}) - \langle t- t^{\prime} , \nabla \psi(t) \rangle = D_{KL}[\pi_{t^{\prime}}(\vz) || \pi_{t}(\vz) ]
% % \end{align}
% % where $\langle \cdot, \cdot \rangle$ indicates a dot product, which reduces to a product for our one-dimensional parameter $t$.

% \paragraph{Variational Representation:}
% \citet{grosse2013annealing} give the following variational representation of a geometric mixture distribution as the solution to a \textsc{kl} divergence minimization
% \begin{align}
%     \pi_{t \cdot T}(\vz) &= \argmin \limits_{r(\vz)} (1-t) \, D_{KL}[ r(\z) || \pi_{0}(\vz)] + \, t \, D_{KL}[  r(\z) || \pi_{T}(\vz)] \label{eq:vrep}
% \end{align}
% While the optimization \eqref{eq:vrep} is over arbitrary  $r(\vz)$, the solution turns out to be a distribution in the exponential family \eqref{eq:exp_fam} with $\log$ likelihood ratio sufficient statistic.  The moment averaged path of \citet{grosse2013annealing} also induces a variational representation using the reverse \textsc{kl} divergence,  although this optimization is only over distributions on the geometric mixture path \eqref{eq:exp_fam} or within a parametric family.  We discuss this distinction in App. \ref{app:mixture_path}. %but this optimization is only over distributions in a parametric family. We discuss this distinction in App. \ref{app:mixture_path}. % Sec. \ and

% %In App. \ref{app:breg_info}, we interpret this result using a general result about Bregman divergences from \citet{Banerjee2005}, where the expected Bregman divergence to a single point $\mu$ in the second argument is minimized by the mean over arguments $\mu = (1-t) \cdot 0 + t \cdot T = t \cdot T$.  With $T=1$, we have $t\cdot T = t$.

% % \subsection{Moment-Averaged Path}
% % \begin{itemize}
% %     \item Introduce conjugate $\psi^{*}$, moments $\eta$, dual divergence $D_{\psi^{*}}$
% %     \item Moments-averaged path of \citet{grosse2013annealing} as variational representation using $D_{\psi^{*}}$
% % \end{itemize}

% % From the convexity of the log partition function $\psi(\tau)$, one can consider its convex conjugate $\psi^{*}$
% % \begin{align}
% % \psi^{*}(\eta) = \sup_{\tau} \tau \cdot \eta - \psi(\tau) \qquad \implies \eta_j &= \frac{\partial \psi}{\partial \tau} \label{eq:conjugate}  \label{eq:conjugate}
% % \end{align}
% % where $\eta = \{ \eta_j \}$ and $\tau = \{ \tau_j \}$ may correspond to $J > 1$ sufficient statistics $\phi(\vz) = \{\phi_j(\vz)\}$.

% % Since $\psi(\tau)$ is convex, its gradient will be unique and increasing at each $\tau$.   We can thus use $\eta = \nabla \psi(\tau)$ as a \textit{dual} way of parameterizing a distribution in the exponential family.  In particular,
% % \begin{align}
% %     \eta_j &= \frac{\partial \psi}{\partial \tau} = \mathbb{E}_{\pi_{\tau}}[ \phi_j(\vz) ] \, \, \forall \, \, j
% % \end{align}
% % which corresponds to the supremum in \eqref{eq:conjugate}.


==> sections/bkup/pre_vaden_thursday_night/2_alpha.tex <==
\section{Interpretations of the $q$-Path}\label{sec:alpha_paths}
We propose to consider the \abstractmean, specified using an order parameter $q$, in place of the geometric average \cref{eq:geopath} for defining \gls{AIS} paths.  In analogy with \cref{sec:alternative_interpretations} above, our generalization is associated with the deformed log mixture, $q$-exponential family, and a variational representation involving the $\alpha$-divergence. %In order to generalize the geometric mixture path, we consider the \abstractmean, parameterized by $q$, in place of the geometric average in \cref{eq:geopath}.
%and moment-averaged paths we consider an abstract mean, parameterized by $\alpha$, in place of the geometric mean used in \cref{eq:geopath}. Analogous to \cref{sec:alternative_interpretations} above, this will result in the deformed log mixture, q-exponential family, and an $\alpha$-divergence variational objective.

% mean parameterized by $\alpha$
% Using variational representations based on the $\alpha$-divergence \cite{amari2007integration, minka2005divergence, amari2016information}, we can follow a similar approach to generalize the geometric and moment-averaged paths.  In particular, these $\alpha$-paths correspond to abstract mixtures using the deformed logarithm and yield a generalization of the exponential family.

%\subsection{Abstract Means}
\paragraph{Abstract Mean}
\begin{wrapfigure}{r}{0.45\textwidth}
    \begin{minipage}{.40\textwidth}
        % \vspace{-10pt}
        \begin{center}
            % \includegraphics[width=\textwidth]{sections/figs/logz_est_alpha_path.pdf}
            \includegraphics[trim={0 0.4cm 0 1.4cm},clip,width=\textwidth]{sections/figs/logz_est_alpha_path.pdf}
        \captionof{figure}{\gls{AIS} estimate of $\log Z_T/Z_0$ by the number of intermediate distributions ($K$) for annealing between $\mathcal{N}(-4,3) \to \mathcal{N}(4,1)$.
        Intermediate $q$ values near 0.9 work better on average.
        }
        \end{center}
        % \vspace{-10pt}
    \end{minipage}\hspace*{.05\textwidth}
    \end{wrapfigure}

We recall a generalization of the mean based on a monotonic function $h(u)$ \cite{de2016mean, amari2007integration}
\begin{align}
\mu_{h}(\{w_i\}, \{u_i\}) = h^{-1} \bigg( \, \sum \limits_{i} w_i \, h(u_i) \, \bigg) \, . \label{eq:abstract_mean}
\end{align}
where $\mu_{h}$ outputs a scalar given a normalized measure $\{ w_i \}$ over a set of non-negative elements $\{ u_i \}$ . In order for the \abstractmean  \textcolor{red}{to be homogenous, i.e. ${\mu_{h}(\{w_i\}, \{c \cdot u_i \}) = c \cdot \mu_{h}(\{w_i\}, \{ u_i \})}$} to have the linear scale-free property ${\mu_{h}(\{w_i\}, \{c \cdot u_i \}) = c \cdot \mu_{h}(\{w_i\}, \{ u_i \})}$ of the geometric and arithmetic mean, \citet{hardy1953} (pg. 68 or \cite{amari2007integration}) show that $h(u)$ must be of the form
\begin{align}
% h_{\alpha}(u) =
% \begin{cases}
%     u^{\frac{1-\alpha}{2}}& \alpha \neq 1 \\
%     \log u \hfill 	&  \alpha = 1
% \end{cases}. \label{eq:alpha_abstract}
h_{q}(u) =
\begin{cases}
    u^{1-q}& q \neq 1 \\
    \log u \hfill 	&  q = 1
\end{cases}. \label{eq:alpha_abstract}
\end{align}
 Several notable examples of the $q$ \abstractmean include the arithmetic mean at $\alpha = -1$, geometric mean at $q \rightarrow 1$, and the $\min$ or $\max$ operation as $q \rightarrow \pm \infty$.  For $q = (1+\alpha)/2$, $h_{q}(u)$ matches the $\alpha$-representation of \citet{amari1982differential}.
% Several notable examples of the $q$ \abstractmean include the arithmetic mean at $\alpha = -1$, geometric mean at $\alpha = 1$, and the $\min$ or $\max$ operation as $\alpha \rightarrow \pm \infty$.  For $q = (1+\alpha)/2$, \eqref{eq:alpha_abstract} matches the $\alpha$-representation of \citet{amari1982differential}.

Using this \abstractmean in place of the geometric mean, we propose defining each intermediate unnormalized density in \gls{AIS} using the $q$-path, % where each mixing parameter $\{ \beta_t \}$ induces a measure $w = \{ 1-\beta_t, \beta_t \}$ over $u = \{ \tpi_0, \tpi_1 \}$.
%Using the abstract mean in place of the geometric mean, we consider this family of $\alpha$-paths in \gls{AIS} by defining each intermediate unnormalized density
% \begin{align}
%     \tilde{\pi}^{(\alpha)}_\beta(\vz) = \begin{cases}\bigg( (1-\beta) \, \tpi_0(\vz)^{\frac{1-\alpha}{2}} + \beta \, \tpi_T(\vz)^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}} & \alpha \neq 1 \\
%      \exp \big( (1-\beta) \, \log \tpi_0(\vz) + \beta \, \log \tpi_T(\vz) \big) & \alpha = 1
%     \end{cases},  \label{eq:alpha_mix}
% \end{align}
\begin{align}
    \tilde{\pi}^{(q)}_t(\vz) = \begin{cases}\bigg( (1-\beta_t) \, \tpi_0(\vz)^{1-q} + \beta_t \, \tpi_T(\vz)^{1-q} \bigg)^{\frac{1}{1-q}} & q \neq 1 \\[1.3ex]
     \exp \big\{ (1-\beta_t) \, \log \tpi_0(\vz) + \beta_t \, \log \tpi_T(\vz) \big\} & q = 1  \\[1.25ex]
    \end{cases},  \label{eq:alpha_mix}
\end{align}
where each mixing parameter $\{ \beta_t \}$ induces $\{ w_i \} = \{ 1-\beta_t , \beta_t \}$ over $\{ u_i \} = \{ f_0, f_T \} $.
%is affine invariant and therefore contains $\ln_q(u)$ as a special case.
%We recover the geometric path for $q \rightarrow 1$ and a mixture between $\tpi_0$ and $\tpi_T$ at $\alpha = 1$. % as seen in \cref{fig:alpha_path}.



%\subsection{Deformed Log Mixture}
\paragraph{Deformed Log Mixture}
In \cref{app:any_h}, we show that any affine transformation of $h_{\alpha}(u)$ yields the same  $\mu_{h}$ in \eqref{eq:abstract_mean} or intermediate $\tilde{\pi}^{(q)}_t(\vz)$ in \eqref{eq:alpha_mix}.
The \textit{deformed}, or $q$-logarithm \cite{naudts2011generalised}, which plays a crucial role in non-extensive thermodynamics \cite{tsallis1988possible, tsallis2009introduction}, is a particular affine transformation, with
\begin{align}
    &\ln_q(u) = \frac{1}{1-q} \big( u^{1-q} - 1 \big) & &\exp_q(u) = \big\{ 1 + (1-q) \, u \big\}_{+}^{\frac{1}{1-q}}
\end{align}
where $\{ x \}_{+} =\textsc{ReLU}[x]= \max\{0, x\}$  ensures $\exp_q(u)$ is non negative. Note that $\lim_{q \to 1} \ln_q(u) = \log u$ and $\lim_{q \to 1} \exp_q(u) = \exp u$,  with $\ln_q (u) = \exp_q^{-1}(u)$.
%\rb{$\{ x \}_{+} = \textsc{ReLU}[x]$? }

We can thus write $\tilde{\pi}^{(\alpha)}_\beta$ as an (unnormalized) $\ln_q$-mixture with mixing weight $\beta_t$,
\begin{align}
    \ln_q \tilde{\pi}^{(q)}_t = (1-\beta_t) \, \ln_q \tpi_0 + \beta_t \ln_q \tpi_T \, ,  \label{eq:ln_q_mix}
\end{align}
which can be verified by direct substitution or with detailed derivations in \textcolor{red}{App. \ref{app:}}


% Defining $q = \frac{1 + \alpha}{2}$, \cref{eq:alpha_mix} can be rewritten
% \begin{align}
%     \tilde{\pi}^{(\alpha)}_\beta = \exp_q\{(1-\beta) \, \ln_q \tpi_0 + \beta \ln_q \tpi_T\},  \label{eq:ln_q_mix}
% \end{align}
% which can be verified by direct substitution and which recovers the geometric path as $q \to 1$. We thus conclude that $\tilde{\pi}^{(\alpha)}_\beta$ can be viewed as a deformed log mixture of $f_0$ and $f_K$.

%\rb{$\ln_q \pi_{t, q}(\vz) = (1-t) \, \ln_q f_0 + t \ln_q f_T - c$ as analogy to $\log$ mixture? with clarification of $c$ (here or later)}

% and in App. \eqref{app:any_h}, we conclude that the $\ln_q$ mixture, as a special case of $h_{\alpha}(u)$, reduces to the $\alpha$-mean $f^{(\alpha)}_t$ in \eqref{eq:alpha_mix}.
%Since $\ln_q(u)$ is a special case of $h_{\alpha}(u)$ for $q = \frac{1+\alpha}{2}$,  we conclude that the $\ln_q$ mixture matches the $\alpha$-mean $f^{(\alpha)}_t$ in \eqref{eq:alpha_mix} (see ).

%\subsection{\texorpdfstring{$q$}{}-Exponential Family}
\paragraph{\texorpdfstring{$q$}{}-Exponential Family}
The $q$-exponential may be used to define a family of distributions \cite{amari2011q, naudts2011generalised} %q-exponential
%\rb{All over the place with notation $Z(\lambda)$ vs. $Z^{(q)}_{t}$ vs. $\pi^{(q)}$ vs. $\psi_q$}
\begin{align}
    \pi_{\lambda}^{(q)}(\z)  &= \pi_0(z) \, \exp_q \big\{ \lambda \cdot \phi(\vz) - \psi_q(\lambda ) \big\} \label{eq:qexp_fam} %\propto \pi_0(z) \, \exp_q \big\{ \lambda \cdot \phi(\vz)  \big\}  % \frac{1}{Z^{(q)}(\lambda)}
\end{align}
which recovers the standard exponential family at $q \to 1$. In \cref{app:q_path} \rb{(Vaden lines 50-54)} we show that the $q$-mixture $\tilde{\pi}^{(\alpha)}_\beta$ \eqref{eq:alpha_mix} can be rewritten in terms of the $q$-exponential family
\begin{align}
    \pi_{t}^{(q)}(\z)  &= \frac{1}{Z^{(q)}_{t}} \tpi_0(\z) \, \exp_q \big\{ \beta_t \cdot \ln_q \frac{\tpi_T(\z)}{\tpi_0(\z)} \big \} %- \psi_q(\beta)  \big\}
    & & Z^{(q)}_{t} = \int \tpi_{t}^{(q)}(\z) \, d\vz \label{eq:z_norm}
\end{align}
with $\phi(\vz) = \ln_q \tpi_T / \tpi_0$ and natural parameter $\beta$.  The expression in \eqref{eq:z_norm} may be used to obtain bounds on the log partition function ratio $\log Z_{T} / Z_0$ as in \gls{BDMC} \cite{grosse2015sandwiching,grosse2016measuring}.

\begin{wrapfigure}{r}{0.40\textwidth}
    \centering
    \begin{minipage}{.34\textwidth}
        \begin{tabular}{ll}
            \toprule
            $q$    &  $Z_{\text{est}}$ ($Z_{\text{true}} = 1$) \\
            \midrule
            0.00 (mix) &  1.0136 $\pm$ 0.0634\\
            0.05 &  1.0105 $\pm$ 0.0569 \\
            0.10 &  1.0198 $\pm$ 0.0576 \\
            \textbf{0.90} &  \textbf{0.9975} $\pm$ \textbf{0.0085} \\
            0.95 &  0.9971 $\pm$ 0.0092 \\
            1.00 (geo) &  0.9967 $\pm$ 0.0094 \\
            \bottomrule
        \end{tabular}
        \captionof{table}{Partition Function Estimates for various $q$ and linearly spaced ${T=100}$. The \abstractmean path parameterized by $q=0.90$ outperforms both the mixture of Gaussians ($q=0$) and geometric ($q=1$) paths in terms of $Z_{\text{err}} = |Z_{\text{est}} - Z_{\text{true}}|$.}\label{tab:logzb}
        % \vspace{-5pt}
    \end{minipage}
\end{wrapfigure}

However, \citet{matsuzoe2019normalization} \cite{suyari2020advantages} highlight the delicate issue of normalization in the $q$-exponential family.   Since 
$\exp_q \{ x + y \} \neq \exp_q \{ x \} \cdot \exp_q \{ y \} $ for $q \neq 1$,
%$\exp_q \{ \beta \cdot \phi - \psi(\beta) \} \neq \frac{1}{\exp_q \{ \psi(\beta) \} } \exp_q \{\beta \cdot \phi \}$ for $q \neq 1$, 
the correspondence between $\log Z_{t} = \psi(\beta_t)$ does not hold for $\ln_q Z^{(q)}_{t} \neq \psi_q(\beta_t) \neq \log Z^{(q)}_{t}$.  We discuss this  distinction in more detail in \rb{App. }, and noting that the $q$-free energy $\psi_q$ has been used to construct a Bregman divergence for the $q$-exponential family in \citet{amari2011q}.


In the next section, we find that the $\ln_q$-mixture or \abstractmean is \textit{also} the solution to an expected divergence minimization problem involving an $f$-divergence.
% $\exp \{ \beta \cdot \phi - \psi(\beta) \} = \frac{1}{\exp \{ \psi(\beta) \} } \exp \{\beta \cdot \phi \}$
%While the


%, and $q$-free energy $\psi_q$ \vm{discuss w/ rob, I don't like this form.}.
% A Bregman divergence may be constructed from the normalization or $q$-free energy $\psi_q$, which yields a variational representation of distributions within the $q$-exponential family as in \eqref{eq:vrep} and \cite{Banerjee2005}.   However, we find that the $\ln_q$- or $\alpha$-mixture is \textit{also} the solution to an expected divergence minimization problem involving an $f$-divergence.

%For distributions within the $q$-family, the mixture in \eqref{eq:ln_q_mix} corresponds to the $q$-geodesic in a dually flat manifold derived from the Bregman divergence associated with the free energy $\psi_q$ \cite{amari2011q}, which similarly corresponds to a mixture of parameters $\lambda_t = (1-t) \lambda_0 + t \lambda_T$.  While this would lead to a similar variational representation as in \eqref{eq:vrep} and \cite{Banerjee2005}, we now demonstrate that the $\ln_q$ mixture can be expressed using an $f$-divergence $D_{\alpha}$.


\subsection{Variational Representation using the \texorpdfstring{$\alpha$}{}-Divergence}
We first recall the definition of the $\alpha$-divergence over unnormalized measures $\tilde{q}$ and $\tilde{p}$ \cite{amari1982differential}.
\begin{align}
D_{\alpha}[\tilde{q} : \tilde{p} ] &= \frac{4}{(1-\alpha^2)} \bigg( \frac{1-\alpha}{2}  \int \tilde{q}(\vz) d\vz +  \frac{1+\alpha}{2}  \int \tilde{p}(\vz) d\vz \big) \label{eq:alpha_div} -\int \tilde{q}(\vz)^{\frac{1-\alpha}{2}} \, \tilde{p}(\vz)^{\frac{1+\alpha}{2}}  d\vz  \bigg)
\end{align}
which is an $f$-divergence \cite{ali1966general} for the generator $f(u) = \frac{4}{1-\alpha^2}\big( \frac{1-\alpha}{2} + \frac{1+\alpha}{2} u -  u^{\frac{1+\alpha}{2}} \big)$ \cite{amari2010divergencefunctions, amari2016information} and closely related to the Tsallis divergence \cite{naudts2011generalised, tsallis2009introduction}.  Note that $\lim \limits_{\alpha \rightarrow 1} D_{\alpha}[\tilde{q} : \tilde{p} ] = D_{KL}[ \tilde{p}:\tilde{q} ]$ and $\lim \limits_{\alpha \rightarrow -1} D_{\alpha}[\tilde{q} : \tilde{p} ] = D_{KL}[\tilde{q} : \tilde{p} ]$.
\footnote{ We extend to unnormalized measures using $D_{\mathrm{KL}}[\tilde{q}(\vz) : \tilde{p}(\vz) ] = D_{KL}[q(\vz) : p(\vz) ] - \int \tilde{q}(\vz) d\vz +  \int \tilde{p}(\vz) d\vz $.}

As in \eqref{eq:vrep}, we consider a path of intermediate distributions $\tpi^{(q)}_{t}$ defined by the variational representation
\begin{align}
%\tpi_{t}^{(q)}(\vz)
\tilde{r}^{*}_{t, \alpha}(\vz) &:= \argmin \limits_{\tilde{r}(\vz)} (1- \beta_t) \, D_{\alpha}[ \tpi_0 (\vz) : \tilde{r}(\vz)  ] + \, \beta_t \, D_{\alpha}[ \tpi_T (\vz) : \tilde{r}(\vz)  ] \label{eq:vrep_alpha}
\end{align}
where the optimization is over \textit{arbitrary} $\tilde{r}(\vz)$.
To find the optimal $\tilde{r}^{*}$ in App. \ref{app:alpha_integration}, we repeat the derivations of \citet{amari2007integration} , where the expected $\alpha$-divergence to a representative $\tilde{r}(\vz)$ is minimized by the abstract mean $\mu_{h_{\alpha}}$ \eqref{eq:abstract_mean}.  For our special case \eqref{eq:vrep_alpha},
\begin{align}
   \tpi_{t}^{(q)}(\vz) =  \tilde{r}^{*}_{t, \alpha}(\vz) = \bigg( (1-\beta_t) \, \tpi_0^{\frac{1-\alpha}{2}} + \beta_t \, \tpi_T^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}}
\end{align}
which corresponds to the $\ln_q$-mixture $\tpi_{t}^{(q)}(\vz)$ as the optimal solution with $q = (1+\alpha) / 2$. % $1 - q = (1-\alpha) / 2$. %, with $q = (1+\alpha) / 2$ or

\paragraph{Moment-Matching Procedure}
%\subsection{Moment-Matching Procedure}
While the solution to the optimization \eqref{eq:vrep_alpha} at $q = 0$ approaches the arithmetic mean, or mixture distribution $\tpi_{t}^{(0)}(\vz) = (1-\beta_t) \, \tpi_0 + \beta_t \, \tpi_1$,  \citet{grosse2013annealing} and \citet{minka2005divergence} (Sec. 3.1-2) have considered similar optimizations restricted to a parametric family of distributions.  For the $\alpha$-divergence in particular, \citet{thang} derives the moment-matching condition
%\citet{thang} \citet{minka2005divergence} Sec. 3.1-2 \textit{within} an exponential family of densities (e.g. Gaussians in Fig. \ref{fig:thang_densities}-\ref{fig:thang_ais}).
\begin{align}
\tilde{r}^{*}_{t, \alpha}(\vz) &:= \argmin \limits_{\tilde{r}(\vz)} (1-\beta_t) \, D_{\alpha}[ \tpi_0 (\vz) : \tilde{r}(\vz)  ] + \, \beta_t \, D_{\alpha}[ \tpi_T (\vz) : \tilde{r}(\vz)  ] \label{eq:vrep_alpha2} \\
\implies \mathbb{E}_{\tilde{r}_{*}}[ \phi(\vz) ] &= (1-\beta_t) \mathbb{E}_{\tpi_0^{\alpha} r_{*}^{1-\alpha} }[ \phi(\vz) ] + \beta_t \, \mathbb{E}_{\tpi_T^{\alpha} \tilde{r}_{*}^{1-\alpha} }[ \phi(\vz) ] \label{eq:moment_matching}
\end{align}
where $\phi(\vz)$ represent the sufficient statistics of an exponential family of interest.    This is reminiscent of a `moment-averaged' path of \citet{grosse2013annealing}, discussed in more detail in App. \ref{app:grosse_alpha}.

However, note that our $q$-path is \textit{more general} than these approaches, since our optimization \eqref{eq:vrep_alpha} is over arbitrary distributions.  Further, instead of a moment matching condition, our closed form expression for $\tpi_{t}^{(q)}(\vz)$ can be directly used as an energy function in \textsc{mcmc} sampling procedures. % such as \gls{HMC} \cite{neal2011mcmc}.

%, now involving the (unnormalized) escort distributions associated with an order of the $\alpha$-divergence (or $q$-family) .


% % \section{\texorpdfstring{$\alpha$}{}-Paths}\label{sec:alpha_paths}
% \section{AIS via Alpha Means}\label{sec:alpha_paths}
%  Using variational representations based on the $\alpha$-divergence \cite{amari2007integration, minka2005divergence, amari2016information}, we can follow a similar approach to generalize the geometric and moment-averaged paths.  In particular, these $\alpha$-paths correspond to abstract mixtures using the deformed logarithm and yield a generalization of the exponential family.

% \subsection{\texorpdfstring{$\alpha$}{}-Paths via Abstract Mean}
% We first recall a generalization of the mean based on any monotonic function $h(u)$, where the mean $\mu_{h}$ takes a normalized measure $\{ w_i \}$ over a set of non-negative elements $\{ u_i \}$ as input and outputs a scalar.   In particular, we let
% \begin{align}
% \mu_{h}(\{w_i\}, \{u_i\}) = h^{-1} \bigg( \, \sum \limits_{i} w_i \, h(u_i) \, \bigg) \, . \label{eq:abstract_mean}
% \end{align}
% However, there is a natural family of functions $h$ to choose, so the abstract mean has the `scale-free' property that for a scalar $c$,  we have $\mu_{h}(\{w_i\}, \{c \cdot u_i \}) = c \cdot \mu_{h}(\{w_i\}, \{ u_i \})$.   \citet{hardy1953} \cite{amari2007integration} show that the only $h(u)$ which have this property are of the form
% \begin{align}
% h_{\alpha}(u) =
% \begin{cases}
%     a \cdot u^{\frac{1-\alpha}{2}} + b \hfill & \alpha \neq 1 \\
%     \log u \hfill 	&  \alpha = 1
% \end{cases} \label{eq:alpha_abstract}
% \end{align}
% Several notable examples of the $\alpha$-abstract mean include the arithmetic mean at $\alpha = -1$, geometric average at $\alpha = 1$, and the $\min$ or $\max$ operation as $\alpha \rightarrow \pm \infty$. In App. \ref{app:any_h}, we show that, for a given $\alpha$, any choice of $a$ and $b$ for $h_{\alpha}(u)$ in  \eqref{eq:alpha_abstract} leads to the same expression for the abstract mean $\mu_{h_{\alpha}}$ \eqref{eq:abstract_mean} .

% We consider this family of $\alpha$-paths for mixing between $f_0$ and $f_T$ in \gls{AIS}, defining each intermediate unnormalized density $f^{(\alpha)}_t$ using the abstract mean
% \begin{align}
%     f^{(\alpha)}_t = \mu_{h_{\alpha}}\big( \{ 1-t, t\}, \{ f_0, f_T \} \big) = \begin{cases}\bigg( (1-t) \, f_0^{\frac{1-\alpha}{2}} + t \, f_T^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}} \hfill \quad \alpha \neq 1 \\
%      \exp \big( (1-t) \, \log f_0 + t \, \log f_T \big) \hfill \quad \alpha = 1 \, ,
%     \end{cases}  \label{eq:alpha_mix}
% \end{align}
% which corresponds to the geometric mixture for $\alpha = 1$.   In the following sections, we interpret the $\alpha$-path for $\alpha \neq 1$ in analogous fashion to the geometric path in \cref{sec:geo}.
% \begin{figure}[t]
%     \centering
%     \subfigure[$\alpha=-1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_00.pdf}}
%     \subfigure[$\alpha=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_09.pdf}}
%     \subfigure[$\alpha=0.8$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_18.pdf}}
%     \subfigure[$\alpha=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_20.pdf}}
%     \caption{Intermediate densities using various $\alpha$-paths between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$, with 10 equally spaced $t$. The $\alpha$-path approaches a mixture of Gaussians with mixing parameter $t$ at $\alpha=-1$, and becomes a geometric mixture parameterized by $t$ at $\alpha=1$.}
%     % \label{fig:foobar}
% \end{figure}
% \subsection{Deformed Logarithm and \texorpdfstring{$\ln_q$}{} Mixture}
% The class of functions $h_{\alpha}(u)$ includes the  \textit{deformed}, or $q$- logarithm \cite{naudts2011generalised}, which plays a crucial role in non-extensive thermodynamics \cite{tsallis1988possible, tsallis2009introduction}.  In particular, we define
% \begin{align}
%     \ln_q(u) = \frac{1}{1-q} \big( u^{1-q} - 1 \big) \qquad \text{and} \qquad \exp_q(u) = \big[ 1 + (1-q) \, u \big]_{+}^{\frac{1}{1-q}}
% \end{align}
% with $\ln_q (u) = \exp_q^{-1}(u)$.  Note that $\ln_q(u)$ is a special case of $h_{\alpha}(u)$ with $a = -b = \frac{1}{1-q}$ and $q = \frac{1+\alpha}{2}$ for $q \neq 1$, with $\lim_{q \to 1} \ln_q(u) = \log u$ as in \eqref{eq:alpha_abstract}.


% Taking the $\ln_q$ mixture of a base distribution $f_0$ and target $f_T$, we can write
% \begin{align}
%   \ln_q \pi_{t, q}(\vz) = (1-t) \, \ln_q f_0 + t \ln_q f_T - c  \label{eq:ln_q_mix}
% \end{align}
% As above and in App. \eqref{app:any_h}, we conclude that the $\ln_q$ mixture, as a special case of $h_{\alpha}(u)$, reduces to the $\alpha$-mean $f^{(\alpha)}_t$ in \eqref{eq:alpha_mix}.
% %Since $\ln_q(u)$ is a special case of $h_{\alpha}(u)$ for $q = \frac{1+\alpha}{2}$,  we conclude that the $\ln_q$ mixture matches the $\alpha$-mean $f^{(\alpha)}_t$ in \eqref{eq:alpha_mix} (see ).

% \subsection{\texorpdfstring{$q$}{}-Exponential Family}
% In analogy with the standard exponential family, the $q$-exponential may used to define a family of distributions \cite{amari2011q, naudts2011generalised}
% \begin{align}
%     \pi_{\lambda,q}(\z)  &= f_0(z) \, \exp_q \big\{ \lambda \cdot \phi(\vz) - \psi_q(\lambda ) \big\}
% \end{align}
% With detailed derivations in \cref{app:q_path}, we show that the $\ln_q$-mixture \eqref{eq:ln_q_mix} (with $c = \psi_q(t) f_0(\z)^{1-q}$) or $\alpha$-mixture
% $f^{(\alpha)}_t$ \eqref{eq:alpha_mix} both reduce to the $q$-exponential family.   In particular, with $\phi(\vz) = \ln_q \frac{f_T}{f_0}$ and natural parameter $t = \lambda$,
% \begin{align}
%     \pi_{t,q}(\z)  &= f_0(\z) \, \exp_q \big\{ t \cdot \ln_q \frac{f_T(\z)}{f_0(\z)} - \psi_q(t)  \big\}
% \end{align}
% A Bregman divergence may be constructed from the normalization or $q$-free energy $\psi_q$, which yields a variational representation of distributions within the $q$-exponential family as in \eqref{eq:vrep} and \cite{Banerjee2005}.   However, we find that the $\ln_q$- or $\alpha$-mixture is \textit{also} the solution to an expected divergence minimization problem involving an $f$-divergence.

% %For distributions within the $q$-family, the mixture in \eqref{eq:ln_q_mix} corresponds to the $q$-geodesic in a dually flat manifold derived from the Bregman divergence associated with the free energy $\psi_q$ \cite{amari2011q}, which similarly corresponds to a mixture of parameters $\lambda_t = (1-t) \lambda_0 + t \lambda_T$.  While this would lead to a similar variational representation as in \eqref{eq:vrep} and \cite{Banerjee2005}, we now demonstrate that the $\ln_q$ mixture can be expressed using an $f$-divergence $D_{\alpha}$.


% \subsection{Variational Representation of the \texorpdfstring{$\alpha$}{}-Divergence}
% We first recall the definition of the $\alpha$-divergence over unnormalized measures $\tilde{q}$ and $\tilde{p}$ \cite{amari1982differential}.
% \begin{align}
% D_{\alpha}[\tilde{q} : \tilde{p} ] &= \frac{4}{(1-\alpha^2)} \bigg( \frac{1-\alpha}{2}  \int \tilde{q}(\vz) d\vz +  \frac{1+\alpha}{2}  \int \tilde{p}(\vz) d\vz \big) \label{eq:alpha_div} -\int \tilde{q}(\vz)^{\frac{1-\alpha}{2}} \, \tilde{p}(\vz)^{\frac{1+\alpha}{2}}  d\vz  \bigg)
% \end{align}
% which is an $f$-divergence \cite{ali1966general} for the generator $f(u) = \frac{4}{1-\alpha^2}\big( \frac{1-\alpha}{2} + \frac{1+\alpha}{2} u -  u^{\frac{1+\alpha}{2}} \big)$ \cite{amari2010divergencefunctions, amari2016information}.  Note that $\lim \limits_{\alpha \rightarrow 1} D_{\alpha}[\tilde{q} : \tilde{p} ] = D_{KL}[ \tilde{p}:\tilde{q} ]$ and $\lim \limits_{\alpha \rightarrow -1} D_{\alpha}[\tilde{q} : \tilde{p} ] = D_{KL}[\tilde{q} : \tilde{p} ]$.
% \footnote{ We extend to unnormalized measures using $D_{\mathrm{KL}}[\tilde{q}(\vz) : \tilde{p}(\vz) ] = D_{KL}[q(\vz) : p(\vz) ] - \int \tilde{q}(\vz) d\vz +  \int \tilde{p}(\vz) d\vz $.}

% As in \cref{eq:vrep}, we consider a path of intermediate distributions $\pi_{t, \alpha}$ defined via the variational representation
% \begin{align}
% \tilde{r}^{*}_{t, \alpha}(\vz) &:= \argmin \limits_{\tilde{r}(\vz)} (1-t) \, D_{\alpha}[ f_0 (\vz) : \tilde{r}(\vz)  ] + \, t \, D_{\alpha}[ f_T (\vz) : \tilde{r}(\vz)  ] \label{eq:vrep_alpha}
% \end{align}
% We repeat these derivations of \citet{amari2007integration} in \cref{app:alpha_integration}, where the expected $\alpha$-divergence to a single $\tilde{r}(\vz)$ is minimized by the abstract mean $\mu_{h_{\alpha}}$ \eqref{eq:abstract_mean}.   For our special case \eqref{eq:vrep_alpha} , the $\alpha$-mean or $\ln_q$-mixture yields the optimal solution $f^{(\alpha)}_t$ to \eqref{eq:vrep_alpha}
% \begin{align}
%   f^{(\alpha)}_t =  \tilde{r}^{*}_{t, \alpha}(\vz) = \bigg( (1-t) \, f_0^{\frac{1-\alpha}{2}} + t \, f_T^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}}
% \end{align}

% \subsection{Moment-Matching Procedure}
% \citet{thang} \citet{minka2005divergence} Sec. 3.1-2 \textit{within} an exponential family of densities (e.g. Gaussians in Fig. \ref{fig:thang_densities}-\ref{fig:thang_ais}).
% \begin{align}
% \tilde{r}^{*}_{t, \alpha}(\vz) &:= \argmin \limits_{\tilde{r}(\vz)} (1-t) \, D_{\alpha}[ f_0 (\vz) : \tilde{r}(\vz)  ] + \, t \, D_{\alpha}[ f_T (\vz) : \tilde{r}(\vz)  ] \label{eq:vrep_alpha2} \\
% \implies \mathbb{E}_{r_{*}}[ \phi(\vz) ] &= (1-t) \mathbb{E}_{f_0^{\alpha} r_{*}^{1-\alpha} }[ \phi(\vz) ] + t \, \mathbb{E}_{f_T^{\alpha} r_{*}^{1-\alpha} }[ \phi(\vz) ] \label{eq:moment_matching}
% \end{align}
% where $\phi(\vz)$ represent the sufficient statistics of the exponential family of interest.    This is reminiscent of a `moment-averaged' path, now involving the (unnormalized) escort distributions associated with an order of the $\alpha$-divergence (or $q$-family) .


==> sections/bkup/pre_vaden_thursday_night/3_info_geo.tex <==
\section{Information Geometric Interpretation}
%%%%%%

Information geometry concerns the study of differential geometric structures over the space of probability distributions $\mathcal{P}$ or unnormalized measures $\mathcal{M}_+$ \cite{amari2016information, nielsen2018elementary}.  In this section, we explore the statistical manifolds induced by the $\alpha$-paths described above. 





%\citet{eguchi1983second} : from divergence to manifold

%In $\mathbb{R}^n$, $D_{\alpha}$ appears to be dually flat ( or \citet{amari2016information} 4.1.2)
%an also try restricting to parametric distributions in the $q$-exponential family
% Following the recipe of \citet{eguchi1983second}, one can use any divergence measure to derive a dual pair of affine connections $\nabla, \nabla^{*}$, which define a covariant derivative operator and parallel transport of vectors between neighboring tangent spaces.   Along with a metric tensor $g$, this defines an \textit{information manifold} $(\mathcal{P}, g, \nabla, \nabla^{*})$. 


% The \textsc{kl} divergence defines a dually flat information manifold $(\mathcal{P}, g^F, \nabla^{1}, \nabla^{-1})$
% \begin{itemize}
% \item \textcolor{red}{Does? } the variational representation \eqref{eq:vrep} corresponds to the distributions along the $\nabla^{(-1)}$ geodesic curve between $f_0$ and $f_T$, parameterized by $t$ (i.e. reverse \textsc{kl}, $\mathbb{E}_{i} D_{\psi}[\theta_i : \theta]$).  (similarly for the reverse \textsc{kl}, with geodesic for connection $\nabla^{(1)}$ )
% \end{itemize}



% $D_{\alpha}$  induces a dually flat structure $(\mathcal{M}_+, g^{?}, \nabla^{(\alpha)}, \nabla^{(-\alpha})$
% \paragraph{Interpreting this:}
 
% \item TO DO : what is the metric $g$?   (Fisher on $\mathcal{M}_+$?) %(simplify \citet{zhang2004divergence} Prop. 7? or even Euclidean (\citet{amari2016information} Sec. 3.6) ))

% \item as above, would hope to interpret $\alpha$-path as a geodesic with respect to $(\mathcal{M}_+, g, \nabla^{\alpha}, \nabla^{-\alpha})$?

% \begin{itemize}
%     \item Can we have dually flat structure on an $\infty$-dim space?
% \begin{itemize}
%     \item \citet{zhang2004divergence} Sec. 3.2 (Ex. 3.2.1, Prop 6) appears to have the same form as the canonical divergence (i.e. $D[\theta : \eta] = \psi(\theta) + \psi^{*}(\eta) - \theta \cdot \eta$)
%     \item \citet{zhang2004divergence} restrict to finite-dim parameter vectors $\theta_p$, $\theta_q$ to define dually flat structure (Prop 7)
%     \item In $\mathbb{R}^n$, $D_{\alpha}$ appears to be dually flat (\citet{felice2019canonical} or \citet{amari2016information} 4.1.2)
% \end{itemize}

% \end{itemize}




% Compare to $\pm \alpha$ connections induced by $D_{KL} = D_{\pm 1}$ as in \citet{nielsen2018elementary}?
% \begin{itemize}
% \item i.e. $\nabla^{\alpha} = \frac{1-\alpha}{2} \nabla^{(-1)} + \frac{1+\alpha}{2} \nabla^{(1)}$
% \item  unsure... ( haven't taken third derivatives)   
% \item  would be nice to be able to unify $\alpha$-paths as $\alpha$-connection induced by $D_{KL} = D_{\pm 1}$
% \end{itemize}


% $\alpha$-path (after normalization) matches the $q$-geodesic in $q$-exponential family (\cite{amari2011geometry} Eq. 65, App. \ref{app:breg_table})
% \begin{itemize}
%     \item even though $q$-geometry is over normalized $\mathcal{P}$, has $g_{ij} = \frac{1}{Z(\text{escort})} g_{ij}^{\text{Fisher}}$ as metric
% \end{itemize}

%Path for $D_{\alpha}$ (in $\mathcal{M}_+$) matches that of $q$-exponential family ( \citet{amari2011geometry}(see \cref{app:breg_table})?
% \begin{itemize}
%     \item $q$-exp family and $\alpha$-mean have same intermediate \textit{unnormalized} densities, different geometry (over different spaces)
%     \item i.e. $q$ geometry constructed using flat divergence over \textit{normalized} distributions (based on normalizer $\psi_q$)
% \end{itemize}

==> sections/bkup/pre_vaden_thursday_night/4_results.tex <==
\section{Experiments}
% comments about code:
% - 'trim={0 1.2cm 0 1cm},clip' crops off labels in favor of latex subcaptions
% - can replace ridge_idx.pdf with idx = enumerate(np.linspace(-1, 1, 21))





% \citet{grosse2013annealing} show the moment-averaged path qualitatively differs from the geometric path (their Fig. 1), and can yield more accurate \gls{AIS} estimates with fewer intermediate distributions (their Fig. 2-3).

%   We hypothesize that different paths may be suitable for various estimation tasks based on the relationship between base and target distributions (uni- vs. multi-modality, heavy tails, etc.)

% Estimation in these plots is based on a moment matching procedure from \citet{minka2005divergence} Sec. 3.1-2 \textit{within} an exponential family of densities (e.g. Gaussians in Fig. \ref{fig:thang_densities}-\ref{fig:thang_ais}).
% \begin{align}
% \tilde{r}^{*}_{t, \alpha}(\vz) &:= \argmin \limits_{\tilde{r}(\vz)} (1-t) \, D_{\alpha}[ f_0 (\vz) : \tilde{r}(\vz)  ] + \, t \, D_{\alpha}[ f_T (\vz) : \tilde{r}(\vz)  ] \label{eq:vrep_alpha2} \\
% \implies \mathbb{E}_{r_{*}}[ \phi(\vz) ] &= (1-t) \mathbb{E}_{f_0^{\alpha} r_{*}^{1-\alpha} }[ \phi(\vz) ] + t \, \mathbb{E}_{f_T^{\alpha} r_{*}^{1-\alpha} }[ \phi(\vz) ] \label{eq:moment_matching}
% \end{align}
% where $\phi(\vz)$ represent the sufficient statistics of the exponential family of interest.    This is reminiscent of a `moment-averaged' path, now involving the (unnormalized) escort distributions associated with an order of the $\alpha$-divergence (or $q$-family) .

% We can now generalize this procedure outside exponential family distributions using the closed form expression for the $\alpha$-mixture. in \eqref{eq:alpha_mix0}, \eqref{eq:alpha_mix}.  It is straightforward to confirm that this satisfies the condition \eqref{eq:moment_matching}.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{sections/figs/gaussian_1d_path.pdf}
%     \caption{
%  Intermediate Gaussian densities using various $\alpha$-paths between $\mathcal{N}(-4, 1)$ and $\mathcal{N}(4,0.2)$, with 25 equally spaced $t$.   %\textbf{Bottom:} Expected log ratios $\mathbb{E}_{z_t} \log \frac{f_T}{f_0}$ along each path (where $\beta = t$).   The integral of this curve can be used to construct \textsc{tvo} bounds.
%  } %, and the point where this curve crosses $0$ corresponds to the Chernoff information $\alpha$.
%     \label{fig:thang_densities}
% \end{figure}



==> sections/bkup/pre_vaden_thursday_night/app/app.tex <==
% \section{Bregman Information (Jensen Gaps \citet{Banerjee2005}}\label{app:breg_info}

\section{The Abstract Mean is Invariant to Affine Transformations} \label{app:any_h}
In this section, we show that $h_{\alpha}(u)$ is invariant to affine transformations. That is, for any choice of $a$ and $b$,
\begin{align}
    h_{\alpha}(u) =
\begin{cases}
    a \cdot u^{\frac{1-\alpha}{2}} + b \hfill & \alpha \neq 1 \\
    \log u \hfill 	&  \alpha = 1
\end{cases} \label{eq:alpha_abstract}
\end{align}
yields the same expression for the abstract mean $\mu_{h_{\alpha}}$. First, we note the expression for the inverse $h^{-1}_{\alpha}(u)$ at $\alpha \neq 1$
\begin{align}
    h^{-1}_{\alpha}(u) = \left(\frac{u - b}{a}\right)^{\frac{2}{1-\alpha}}.
\end{align}
Recalling that $\sum_i w_i = 1$, the abstract mean then becomes
\begin{align}
    \mu_{h_{\alpha}}(\{w_i\}, \{u_i\}) &= h_{\alpha}^{-1}\left(\sum_i w_i h_{\alpha}(u_i) \right) \\
    &= h_{\alpha}^{-1}\left(a \left(\sum_i w_iu_i^{\frac{1-\alpha}{2}}\right) + b \right) \\
    &=\bigg(\sum_i w_i u_i^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}}
\end{align}
which is independent of both $a$ and $b$. The $\alpha$-representation \cite{amari2007integration,amari2016information} appears as a special case with $a=1$ and $b=0$, while the deformed logarithm $\ln_q$ corresponds to $a=-b = \frac{1}{1-q}$ for $q=\frac{1+\alpha}{2}$.
% prev
% \begin{align}
%     y = h_{\alpha}(u) &= a \cdot u^{\frac{1-\alpha}{2}} + b \\
%     \frac{y - b}{a} &= u^{\frac{1-\alpha}{2}} \\
% \end{align}




% % \section{Bregman Information (Jensen Gaps \citet{Banerjee2005}}\label{app:breg_info}

% \section{The Abstract Mean is Invariant to Affine Transformations in $h_{\alpha}(u)$ } \label{app:any_h}
% In this section, we show that any choice of $a$ and $b$ for $h_{\alpha}(u)$ \eqref{eq:alpha_abstract} yields the same expression for the abstract mean $\mu_{h_{\alpha}}$. First, we note the expression for the inverse $h^{-1}_{\alpha}(y)$ at $\alpha \neq 1$
% \begin{align}
%     h^{-1}_{\alpha}(u) = \left(\frac{u - b}{a}\right)^{\frac{2}{1-\alpha}}.
% \end{align}
% Recalling that $\sum_i w_i = 1$, the abstract mean then becomes
% \begin{align}
%     \mu_{h_{\alpha}}(\{w_i\}, \{u_i\}) &= h_{\alpha}^{-1}\left(\sum_i w_i h_{\alpha}(u_i) \right) \\
%     &= h_{\alpha}^{-1}\left(a \left(\sum_i w_iu_i^{\frac{1-\alpha}{2}}\right) + b \right) \\
%     &=\bigg(\sum_i w_i u_i^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}}
% \end{align}
% which is independent of both $a$ and $b$.
% The $\alpha$-representation \cite{amari2007integration,amari2016information} appears as a special case with $a=1$ and $b=0$, while the deformed logarithm $\ln_q$ corresponds to $a=-b = \frac{1}{1-q}$. For the abstract mean of two unnormalized densities $\{ f_0, f_T \}$ with weights $\{ 1-t, t \}$, we obtain the $\alpha$-mean in \eqref{eq:alpha_mix0}.

% % prev
% % \begin{align}
% %     y = h_{\alpha}(u) &= a \cdot u^{\frac{1-\alpha}{2}} + b \\
% %     \frac{y - b}{a} &= u^{\frac{1-\alpha}{2}} \\
% % \end{align}




% \prev
\section{Derivation of Path $q$-Family}\label{app:q_path}
While the exponential family has the convenient property that $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \}  $, this is not true for $\exp_{\alpha}\{ x + y \}$.  The $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
\begin{align}
    \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ t \cdot \phi(\vz) - \psi_q  \big\} \label{eq:lnq_fam}
\end{align}
where $\psi_q$ enforces the normalization.  As \citet{amari2011q} show that $\psi_q(t)$ is convex in the parameter $t$, we can write \eqref{eq:lnq_fam} in a form suggestive of the conjugate function $\psi_q^{*}$,
\begin{align}
    \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  t \cdot \phi(\vz) - \psi_q(t) \, .
\end{align}
We now derive the $q$-exponential family from the $\ln_q$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.

\begin{proof}  To normalize by subtracting the $q$-free energy $\psi_q$, we must also multiply by a factor of $\pi_0^{1-q}$.
\begin{align*}
    \pi_{t,q}(\z) &=  \exp_q \left\{ (1-t) \ln_q \pi_0(\z) + t \ln_q \pi_1(\z)  - \psi_q \cdot \pi_0(\z)^{1-q} \right\} \\
    &= \left[ 1 + (1-q) \left( \ln_q \pi_0(\z) + t \left( \ln_q \pi_1(\z) - \ln_q \pi_0(\z) \right)\right)- (1-q) \psi_q \cdot \pi_0(\z)^{1-q} \right]_{+}^{\frac{1}{1-q}} \\
    &= \left[ 1 + (1-q) \frac{1}{1-q} \left( \pi_0(\z)^{1-q} - 1  + t \big( \pi_1(\z)^{1-q} - 1 - \pi_0(\z)^{1-q} + 1 \big)\right) - (1-q) \psi_q \cdot \pi_0(\z)^{1-q}   \right]_{+}^{\frac{1}{1-q}} \\
  &= \left[ 1 +  \pi_0(\z)^{1-q} - 1  + t \bigg( \pi_1(\z)^{1-q}  - \pi_0(\z)^{1-q} \bigg)  - (1-q) \psi_q \cdot \pi_0(\z)^{1-q}  \right]_{+}^{\frac{1}{1-q}} \\
  &= \left[  \pi_0(\z)^{1-q}  + t \, \pi_1(\z)^{1-q} - t \, \pi_0(\z)^{1-q}   - (1-q) \psi_q \cdot \pi_0(\z)^{1-q} \right]_{+}^{\frac{1}{1-q}} \\
    &= \left[  \pi_0(\z)^{1-q} \left(1 +  t \, \bigg(\frac{\pi_1(\z)}{\pi_0(\z)}\bigg)^{1-q} - t - (1-q) \psi_q \right)    \right]_{+}^{\frac{1}{1-q}} \\
    &= \pi_0(\z) \left[ 1 +  (1-q)  \cdot \left( t \cdot \ln_q \frac{\pi_1(\z)}{\pi_0(\z)}  - \psi_q \right) \right]_{+}^{\frac{1}{1-q}} \\
    &= \pi_0(z) \, \exp_q \big\{ t \cdot \ln_q \frac{\pi_1(\z)}{\pi_0(\z)} - \psi_q  \big\}
\end{align*}
\text{ which matches \eqref{eq:lnq_fam}.}
\end{proof}

\section{\texorpdfstring{$\alpha$}{}-Integration}\label{app:alpha_integration}
\vm{vaden to rewrite to handle +/- 1 cases separately and make notation consistent w/ below}
\citet{amari2007integration} show that the $\alpha$-mixture $\pi_{\alpha_t}$ minimizes the expected divergence to a single point.
\begin{align}
\pi_{\alpha_t}(\vz) &= \argmin \limits_{r(\vz)} \sum \limits_{i=1}^{N} w_i \, D_{\alpha}[p_i (\vz) : r(\vz) ] \label{eq:amari_vrep} \\
\text{where} \quad \pi_{\alpha_t}(\vz) &= \big( \sum \limits_{i=1}^{N} w_i \, p_i (\vz)^{\frac{1-\alpha}{2}}     \big)^{\frac{2}{1-\alpha}} \label{eq:alpha_mix_app}
\end{align}
\begin{proof}
\begin{align}
\frac{d}{dr} \sum \limits_{i=1}^{N} w_i \, D_{\alpha}[p_i (\vz) : r(\vz) ] &= \frac{d}{dr} \frac{4}{1-\alpha^2} \sum \limits_{i=1}^{N} w_i \big( -\int p_i(\vz)^{\frac{1-\alpha}{2}}\, r(\vz)^{\frac{1+\alpha}{2}} d\vz  +  \frac{1+\alpha}{2} \int r(\vz) d\vz \big) \\
0 &=\frac{4}{1-\alpha^2} \big( -{\frac{1+\alpha}{2}} \sum \limits_{i=1}^{N} w_i  \, p_i(\vz)^{\frac{1-\alpha}{2}}\, r(\vz)^{\frac{1+\alpha}{2}-1} + \frac{1+\alpha}{2} \big) \\
- \frac{2}{1-\alpha} &= -\frac{2}{1-\alpha} \sum \limits_{i=1}^{N} w_i  \, p_i(\vz)^{\frac{1-\alpha}{2}}  r(\vz)^{-\frac{1-\alpha}{2}} \\
 r(\vz)^{\frac{1-\alpha}{2}} &= \sum \limits_{i=1}^{N} w_i  \, p_i(\vz)^{\frac{1-\alpha}{2}} \\
  r(\vz) &= \bigg(\sum \limits_{i=1}^{N} w_i  \, p_i(\vz)^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}}
\end{align}
\end{proof}
%The function $f_{\alpha}(p) = \frac{2}{1-\alpha} \, p^{\frac{1-\alpha}{2}}$ is known as the $\alpha$-representation of a distribution $p$ \cite{amari2016information}.
This result is similar to a general result about Bregman divergences in \citet{Banerjee2005} Prop. 1, although $D_{\alpha}$ is not a Bregman divergence.

\subsection{Arithmetic Mean ($\alpha = -1$)}\label{app:mixture_path}
\newcommand{\pa}{\pi_0}%{p_a}
\newcommand{\pb}{\pi_1}%{p_b}
\newcommand{\opt}{r}%{q}
%\section{Relationship between \texorpdfstring{$\alpha$}{}-mean path and Grosse's moment averaging path}\label{app:grosse_alpha}
The moment-averaging path from Grosse\cite{grosse2013annealing} is \textit{not} a special case of the $\alpha$-mean path of Amari \cite{amari2007integration}. This is because while they both minimize a convex combination of reverse KL's, Grosse minimize in the constrained space of \textit{minimal exponential families}, while Amari optimizes over \textit{all} normalized distributions.

More formally, consider minimizing the functional
\begin{align}
    J[\opt] &= (1 - \beta)\int \pa(z) \log \frac{\pa(z)}{\opt(z)} dz + \beta \int \pb(z) \log \frac{\pb(z)}{\opt(z)} dz \\
         &= \text{const} - \int \left[(1 - \beta) \pa(z) + \beta \pb(z) \right] \log \opt(z) dz \label{eq:functional}
\end{align}
We will show how Grosse and Amari minimize \ref{eq:functional}.



\paragraph{Grosse's solution}
Grosse constrains $\opt(z) = \frac{1}{Z(\eta)} h(z) \exp (\eta^T g(z))$ to be a (minimal) exponential family model and minimizes \ref{eq:functional} w.r.t $\opt$'s  natural parameters $\eta$ (cf. \cite{grosse2013annealing} appendix 2.2):
\begin{align}
    \eta^*_i &= \argmin_\eta J(\eta) \\
    &= \argmin_\eta \left(- \int \left[(1 - \beta) \pa(z) + \beta \pb(z) \right] \left[ \log h(z) + \eta^T g(z) - \log Z(\eta) \right] dz \right)\\
    &= \argmin_\eta \left(\log Z(\eta) - \int \left[(1 - \beta) \pa(z) + \beta \pb(z) \right] \eta^T g(z) dz  + \text{const}\right)
\end{align}
where the last line follows because $\pa(z)$ and $\pb(z)$ are assumed to be correctly normalized. Then to arrive at the moment averaging path, we compute the partials $\frac{\partial J(\eta)}{\partial \eta_i}$ and set to zero:
\begin{align}
    \frac{\partial J(\eta)}{\partial \eta_i} &= \E_{\opt}[g_i(z)] - (1 - \beta)\E_{\pa}[g_i(z)] - \beta \E_{\pb}[g_i(z)] = 0 \\
    \E_{\opt}[g_i(z)] &= (1 - \beta)\E_{\pa}[g_i(z)] - \beta \E_{\pb}[g_i(z)]
\end{align}
where we have used the exponential family identity $\frac{\partial \log Z(\eta)}{\partial \eta_i} = \E_{\opt_{\eta}}[g_i(z)]$ in the first line.




\paragraph{Amari's solution}
Instead of optimizing in the space of minimal exponential families, Amari instead adds a Lagrange multiplier to \ref{eq:functional} and optimizes $\opt$ directly (cf. \cite{amari2007integration} eq. 5.1 - 5.12)
\begin{align}
    {\opt}^* &= \argmin_{\opt} J'[\opt] \\
    &= \argmin_{\opt} J[\opt] + \lambda \left(1 - \int \opt(z) dz\right) \label{eq:lagrange}
\end{align}
\ref{eq:lagrange} can be minimized using the Euler-Lagrange equations or using the identity
\begin{align}
    \frac{\delta f(x)}{\delta f(x')} = \delta(x - x')\label{eq:delta_eq}
\end{align}
from \cite{meng2004introduction}. We compute the functional derivative of $J'[\opt]$ using \ref{eq:delta_eq} and solve for $q$:
\begin{align}
    \frac{\delta J'[\opt]}{\delta \opt(z)}=&- \int \big[(1 - \beta) \pa(z') + \beta \pb(z') \big] \frac{1}{\opt(z')} \frac{\delta \opt(z')}{\delta \opt(z)} dz' - \lambda \int \frac{\delta \opt(z')}{\delta \opt(z)} dz' \\
    =&- \int \big[(1 - \beta) \pa(z') + \beta \pb(z') \big] \frac{1}{\opt(z')} \delta(z - z') dz' - \lambda \int \delta(z - z') dz' \\
    =&- \big[(1 - \beta)\pa(z) + \beta \pb(z)\big] \frac{1}{\opt(z)} - \lambda = 0
\end{align}
Therefore
\begin{align}
    \opt(z) \propto \big[(1 - \beta)\pa(z) + \beta \pb(z)\big],
\end{align}
which corresponds to the alpha path at $\alpha = -1$. Thus, while both Amari and Grosse start with the same objective, they arrive at different optimum because they optimize over different spaces.




==> sections/bkup/pre_vaden_thursday_night/app/breg_table.tex <==
\section{Comparison of Exponential Family and $q$-Exponential Family}\label{app:breg_table}
\begin{table}[h]
\centering
\caption{\label{tab:properties}}
\begin{tabular}{p{2cm} p{6.1cm} p{6.5cm}} % \cmidrule(r){1-1}
  \cmidrule(lr){2-2} \cmidrule(l){3-3} \\[.25ex]
 & Exponential Family ($q=1$) & $q$-Exponential Family \\ \midrule
Definition & $\pi_{\beta}(\z) = \pi_0(\z) \, \exp \{ \beta \cdot \phi(\z) - \psi(\beta) \}$  & $\pi_{\lambda}(\z) = \pi_0(\z) \, \exp_q \{ \lambda \cdot \phi(\z) - \psi_q(\lambda) \} $ \\[2ex]
Free Energy & $\psi(\beta)  = \ln Z_{\beta} $ & $\psi_q(\lambda)$ \\[2ex]
Escort Dist. & $\Pi_{\beta, 1} =  \pi_0(\z)^{1-1} \, \pi_{\beta}(\z)^1 =  \pi_{\beta}(\z)  $ & $ \Pi_{\lambda,q} = \dfrac{1}{z_{q}(\lambda)} \pi_0(\z)^{1-q} \, \pi_{\lambda,q}(\z)^q $ \\[2ex]
Dual Params 		& $\dfrac{\partial \psi(\beta)}{\partial \beta^j} = \eta^j =  \mathbb{E}_{\pi_{\beta}}[\phi_j(\z)]$    \, (standard)		& $\dfrac{\partial \psi_q(\lambda)}{\partial \lambda^j} =\eta^j_q =\mathbb{E}_{\Pi_{\lambda,q}}[\phi_j(\z)] $ \, (escort) \\[2ex]
Bregman Div. & $D_{\psi}[\beta^{\prime} : \beta ] = D_{KL}[ \pi_{\beta} || \pi_{\beta^{\prime}} ] $ & $D_{\psi_q}[\lambda^{\prime} : \lambda ] = \mathbb{E}_{\Pi_{\lambda, q} }[ \ln_q \dfrac{\pi_{\lambda,q}}{\pi_0} - \ln_q \dfrac{\pi_{\lambda^{\prime},q}}{\pi_0}] $ \\[2ex]
& $\phantom{D_{\psi}[\beta^{\prime} : \beta ]} = \mathbb{E}_{\pi_{\beta}} [ \ln \pi_{\beta} - \ln \pi_{\beta^{\prime}} ]$ &  \\[2ex]
Conjugate $\psi^{*}$ & $\psi^{*}(\eta) = D_{\psi}[\pi_0 ||  \pi_{\beta_{\eta}}] =D_{KL}[\pi_{\beta_{\eta}}||\pi_0 ] $ & $\psi_q^{*}(\eta) = D_{\psi_q}[\pi_0 ||\pi_{\lambda_{\eta},q}] = \mathbb{E}_{\Pi_{\lambda, q} }[ \ln_q \dfrac{\pi_{\lambda_{\eta},q}}{\pi_0} ] $\\[2ex] 
& & $\phantom{\psi_q^{*}(\eta) = } \hfill = \dfrac{1}{1-q}\bigg(\dfrac{1}{z_q(\lambda)} -1 \bigg) $ \\[3.5ex] \\
Neg. Entropy & $\psi^{*}(\eta) = \mathbb{E}_{\pi_{\beta_{\eta}}}[ \log \pi_{\beta_{\eta}} ] $\footnotesize \quad (if $\pi_0 =$uniform)& $\psi_q^{*}(\eta) = \mathbb{E}_{\Pi_{\lambda, q}}[ \ln_q \pi_{\lambda_{\eta},q} ] $  \footnotesize \quad (if $\pi_0 = $uniform) \\[3ex]
\small Dual Definition & $\pi_{\beta}(\z) = \pi_0(\z) \exp \{ \beta \, ( \phi(\z) - \eta ) + \psi^{*}(\eta) \}$  & $\pi_{\lambda}(\z) = \pi_0(\z)\exp_q \{ \lambda \, ( \phi(\z) - \eta_q ) + \psi_q(\lambda) \}$ \\
\bottomrule
\end{tabular}
\end{table}


==> sections/bkup/pre_vaden_thursday_night/app/vm_naudts_paths.tex <==
\section{Derivation of Path $q$-Family}\label{app:q_path}
\vm{This longer derivation is necessary to establish relationship between two q-exp fam forms and allow for tvo/ti trick. Might also be better to save for full paper and revert to prev}
With normalization, the $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
\begin{align}
    \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ \eta \cdot \phi(\vz) - \psi_q(\eta)  \big\} \label{eq:lnq_fam_form1}
\end{align}
which is suggestive of the convex conjugate for $\psi_q$ via
\begin{align}
    \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  \eta \cdot \phi(\vz) - \psi_q(\eta)
\end{align}
We now derive the $q$-exponential family from the $\alpha$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.

\begin{proof}
\begin{align}
    \pi_{\alpha, \beta}(z) &\propto \bigg[(1 - \beta) \pi_0^{1 - \alpha} + \beta\pi_1^{1 - \alpha}\bigg]^\frac{1}{1 - \alpha}\\
    &= \bigg[\pi_0^{1 - \alpha} + \beta\big(\pi_1^{1 - \alpha} - \pi_0^{1 - \alpha}\big)\bigg]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + \beta\left(\left(\frac{\pi_1}{\pi_0}\right)^{1 - \alpha} - 1\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + (1-\alpha)\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \exp_\alpha\left[\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right].
\end{align}
Defining $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$ and normalizing, we arrive at
\begin{align}
    \pi_{\alpha, \beta}(z) = \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \quad
    Z_\alpha(\beta) &:= \int dz \pi_0 \exp_\alpha\left[\beta \phi(\vz) \right].\label{eq:lnq_fam_form2}
\end{align}

To get \cref{eq:lnq_fam_form2} into the standard $q$-exponential family form, we define
\begin{align}
    \psi_\alpha := \ln_\alpha^* \left(Z_\alpha(\beta)\right) \label{eq:psi_alpha}
\end{align}
and rewrite \cref{eq:lnq_fam_form2} using \cref{eq:q_exp_prod}
\begin{align}
    \pi_{\alpha, \beta}(z) &= \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \\
    &= \frac{\pi_0}{\exp^*_\alpha\left(\psi_\alpha\right)}\exp_\alpha\left(\beta \phi(\vz) \right) & \text{Using  \cref{eq:psi_alpha}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha\right) \exp_\alpha\left(\beta \phi(\vz)\right) & \text{Using $\exp^*_\alpha(u) = 1/\exp_\alpha(-u)$}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \bigg(1 - (1 - \alpha) \psi_\alpha\bigg)\beta\phi(\vz)\right) & \text{Using \cref{eq:q_exp_prod}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \eta \phi(\vz)\right)
\end{align}
where we have defined
\begin{align}
    \eta := \beta \cdot \big(1 - (1 - \alpha) \psi_\alpha\big).
\end{align}
\end{proof}



\section{Alternative Derivation}
Note that $\exp_q \{ x + y \} = \exp_q \{ y \} \cdot \exp_q \{ \frac{x}{1 + (1-q) y}  \}$ from \textcolor{red}{Vaden's theorem below.}, instead of $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $ for the standard exponential.  This implies that
\begin{align}
\pi_{q,\beta} = \pi_0 \, \exp_q \{ \beta \cdot \phi(\vz) - \psi_q \} &= \pi_0 \, \exp_q\{ -\psi_q \} \exp_q \{ \frac{\beta}{1+(1-q)(-\psi_q)} \cdot \phi(\vz) \} 
\end{align}
Our goal is to express $\pi_{q,\beta}(\vz)$ using a normalization constant $Z$ instead of the $q$-free energy $\psi_q(\beta)$.  While the exponential family allows us to freely move between  $\log Z_{\beta}$
and $\psi(\beta)$, in the $q$-exponential case, we must adjust the parameters.   Defining
%To (w/ $\eta, \beta$ switched) match Naudts, let : }
\begin{align}
 \eta &= \frac{\beta}{1+(1-q)(-\psi_q)} \\
Z_q(\eta) &= \frac{1}{\exp_q \{-\psi_q \}} := \exp_{q}^{*}\{ -\psi_q\} \\
\end{align}
we obtain a new parameterization of the $q$-exponential family, using parameters $\eta$ and multiplicative normalization constant $Z_q(\eta)$, as
\begin{align}
 \pi_{q,\beta} =  \pi_{q,\eta} &=  \frac{1}{Z_q(\eta)} \exp_{q} \{ \eta \cdot \phi(\vz) \}
\end{align}
See \citet{matsuzoe2019normalization} for more detailed discussion of normalization in deformed exponential families.


==> sections/bkup/pre_vaden_thursday_night/app/vm_q_sum_prod.tex <==
\section{Sum and product identities for q-exponentials}\label{app:q_sum_product}
While the exponential family has the convenient property that $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $, this is not true for $\exp_{\alpha}\{ x + y \}$. We therefore derive two lemmas for q-exponentials which will be useful in obtaining the $q$-exponential family. We will prove both statements by induction and simplify notation by defining $\bar{q} := 1 - q$.

\begin{lemma}
    Sum identity
    \begin{align}
        \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
    \end{align}
    \begin{proof}
        The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$. Assuming \cref{eq:q_exp_sum} holds for $N$,
        \begin{align}
            \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \bigg[ 1 + \bar{q} \sum_{n=1}^{N+1} x_n \bigg]^{1/\bar{q}} \\
                                                    &= \bigg[ 1 + \bar{q} \left(\sum_{n=1}^{N} x_n\right) + \bar{q}x_{N+1} \bigg]^{1/\bar{q}} \\
                                                    &= \bigg[\left( 1 + \bar{q} \sum_{n=1}^{N} x_n \right) \left(1 + \bar{q}\frac{x_{N+1}}{1 + \bar{q} \sum_{n=1}^{N} x_n}\right) \bigg]^{1/\bar{q}} \\
                                                    &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + \bar{q} \sum_{n=1}^{N} x_n} \right)\\
                                                    &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + \bar{q}\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
        \end{align}
    \end{proof}
\end{lemma}

\begin{lemma}
    Product identity
    \begin{align}
        \prod_{n=1}^N \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1 - q)x_i\right)\right)\label{eq:q_exp_prod}
    \end{align}
    \begin{proof}
        The base case ($N=1$) is satisfied using the convention $\prod_{i=a}^bx_i = 1$ if $b < a$. Assuming \cref{eq:q_exp_prod} holds for $N$, we will show the $N+1$ case. To simplify notation we define $y_N:=\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q}x_i\right)$. Then
    \begin{align}
        \prod_{n=1}^{N+1} \exp_q(x_n) &= \exp_q(x_{1})\left(\prod_{n=2}^{N+1}\exp_q(x_n)\right)\\
        &= \exp_q(x_{0})\left(\prod_{n=1}^{N}\exp_q(x_n)\right) & \text{(reindex $n \to n - 1)$}\\
        &=\exp_q(x_{0})\exp_q(y_N) & \text{(inductive hypothesis)}\\
        &= \bigg[\left(1 + \bar{q} \cdot x_{0}\right)\left(1 + \bar{q} \cdot y_N\right) \bigg]^{1/\bar{q}}\\
        &= \bigg[1 + \bar{q} \cdot x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)\bar{q} \cdot y_N \bigg]^{1/\bar{q}}\\
        &= \bigg[1 + \bar{q} \bigg(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)y_N\bigg) \bigg]^{1/\bar{q}}\\
        &= \exp_q \left(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)y_N\right)
    \end{align}
    Next we use the definition of $y_N$ and rearrange
    \begin{align}
        &= \exp_q \left(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)\left(x_1 + x_2(1 + \bar{q} \cdot x_1) + ... + x_N \cdot \prod_{i=1}^{N-1}(1 + \bar{q} \cdot x_i)\right)\right)\\
        &= \exp_q\left(\sum_{n=0}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q} x_i\right)\right).
    \end{align}
    Then reindexing $n \to n + 1$ establishes
    \begin{align}
        \prod_{n=1}^{N+1} \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N+1}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q}x_i\right)\right).
    \end{align}
\end{proof}
\end{lemma}

\section{Derivation of Path $q$-Family}\label{app:q_path}
\vm{This longer derivation is necessary to establish relationship between two q-exp fam forms and allow for tvo/ti trick. Might also be better to save for full paper and revert to prev}
With normalization, the $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
\begin{align}
    \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ \eta \cdot \phi(\vz) - \psi_q(\eta)  \big\} \label{eq:lnq_fam_form1}
\end{align}
which is suggestive of the convex conjugate for $\psi_q$ via
\begin{align}
    \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  \eta \cdot \phi(\vz) - \psi_q(\eta)
\end{align}
We now derive the $q$-exponential family from the $\alpha$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.

\begin{proof}
\begin{align}
    \pi_{\alpha, \beta}(z) &\propto \bigg[(1 - \beta) \pi_0^{1 - \alpha} + \beta\pi_1^{1 - \alpha}\bigg]^\frac{1}{1 - \alpha}\\
    &= \bigg[\pi_0^{1 - \alpha} + \beta\big(\pi_1^{1 - \alpha} - \pi_0^{1 - \alpha}\big)\bigg]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + \beta\left(\left(\frac{\pi_1}{\pi_0}\right)^{1 - \alpha} - 1\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + (1-\alpha)\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \exp_\alpha\left[\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right].
\end{align}
Defining $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$ and normalizing, we arrive at
\begin{align}
    \pi_{\alpha, \beta}(z) = \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \quad
    Z_\alpha(\beta) &:= \int dz \pi_0 \exp_\alpha\left[\beta \phi(\vz) \right].\label{eq:lnq_fam_form2}
\end{align}

To get \cref{eq:lnq_fam_form2} into the standard $q$-exponential family form, we define
\begin{align}
    \psi_\alpha := \ln_\alpha^* \left(Z_\alpha(\beta)\right) \label{eq:psi_alpha}
\end{align}
and rewrite \cref{eq:lnq_fam_form2} using \cref{eq:q_exp_prod}
\begin{align}
    \pi_{\alpha, \beta}(z) &= \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \\
    &= \frac{\pi_0}{\exp^*_\alpha\left(\psi_\alpha\right)}\exp_\alpha\left(\beta \phi(\vz) \right) & \text{Using  \cref{eq:psi_alpha}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha\right) \exp_\alpha\left(\beta \phi(\vz)\right) & \text{Using $\exp^*_\alpha(u) = 1/\exp_\alpha(-u)$}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \bigg(1 - (1 - \alpha) \psi_\alpha\bigg)\beta\phi(\vz)\right) & \text{Using \cref{eq:q_exp_prod}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \eta \phi(\vz)\right)
\end{align}
where we have defined
\begin{align}
    \eta := \beta \cdot \big(1 - (1 - \alpha) \psi_\alpha\big).
\end{align}
\end{proof}

